Efficient Optimistic Exploration in Linear-Quadratic Regulators via Lagrangian Relaxation

We study the exploration-exploitation dilemma in the linear quadratic regulator (LQR) setting. Inspired by the extended value iteration algorithm used in optimistic algorithms for finite MDPs, we propose to relax the optimistic optimization of \ofulq and cast it into a constrained \textit{extended} LQR problem, where an additional control variable implicitly selects the system dynamics within a confidence interval. We then move to the corresponding Lagrangian formulation for which we prove strong duality. As a result, we show that an $\epsilon$-optimistic controller can be computed efficiently by solving at most $O\big(\log(1/\epsilon)\big)$ Riccati equations. Finally, we prove that relaxing the original \ofu problem does not impact the learning performance, thus recovering the $\tilde{O}(\sqrt{T})$ regret of \ofulq. To the best of our knowledge, this is the first computationally efficient confidence-based algorithm for LQR with worst-case optimal regret guarantees.

==> app_aux_proofs_lipschitz.tex <==
% !TEX root = main.tex

\section{Proof of Lem.~\ref{le:smoothness.D} and Cor.~\ref{co:smoothness.avg.cost.control}}\label{sec:app.aux.proof.lipschitz}

In this section, we proceed with the same notations as in Sec.~\ref{sec:app.proof.duality}. The proof of Lem.~\ref{le:smoothness.D} is decomposed in several steps: \textbf{1)} we show that $\mathcal{M}_{\wt{D}}$ is a subset of $\mathcal{M}$ over which the riccati equation associated with $\mathcal{D}$ behaves 'nicely', that is for any $(\mu,\nu) \in \mathcal{M}_L$, $\|K_{\mu,\nu}\|_2$ is finite, $A_c^\mu = A + \wt{B} K_{\mu,\nu}$ is stable enough and $\mathcal{D}$ is Lipschitz. \textbf{2)} Stability, bounded control and Lipschitz guarantees ensures $(\mu,\nu) \rightarrow P_{\mu,\nu}$ to be Lispchitz and further $(\mu,\nu) \rightarrow K_{\mu,\nu}$ to be Lispchitz. \textbf{3)} Lipschitz continuity of $(\mu,\nu) \rightarrow K_{\mu,\nu}$ translates in Lispchitz continuity of $(\mu,\nu) \rightarrow \nabla \mathcal{D}(\mu,\nu)$.\\
Finally, we conclude with the proof of Cor.~\ref{co:smoothness.avg.cost.control} which relies on those intermediate results.



\subsection{Step 1)}
\begin{proposition}\label{p:stable.bounded.set}
	For all $(\mu,\nu) \in \mathcal{M}_{\wt{D}}$, let $K_{\mu,\nu}$ be the optimal control and $A^c_{\mu,\nu} = A + \wt{B} K_{\mu,\nu}$ be the optimal closed-loop matrix. Let $K^{u}_{\mu,\nu}$, $K^{w}_{\mu,\nu}$ be its control and perturbation sub-matrix respectively. Let $\wt{\kappa} = \wt{D}/\lambda_{\min}(H)$, then,
	\begin{equation*}
	\begin{aligned}
	& \|K_{\mu,\nu}\|_2 \leq \|K_{\mu,\nu} \|_F \leq \sqrt{\wt{\kappa}}; \\
	& \mathcal{D}^\prime_\mu(\mu,\nu) \leq l_\mu; \quad\quad | \mathcal{D}^\prime_\nu(\mu,\nu) | \leq l_\nu; \\
	& \| d_\mu P_{\mu,\nu} \|_2 \leq l_\mu; \quad\quad \| d_\nu P_{\mu,\nu} \|_2 \leq l_\nu; \\
	\end{aligned}
	\end{equation*}
	where 
	\begin{equation*}
	l_\mu =\wt{\kappa}^2 \max\big(\wt{\kappa}, \|V^{-1}\|_2 \big); \quad\quad l_\nu =\max\Big( \wt{\kappa}\big(1 + \|K_0\|_2^2\big), \big( \epsilon_0^{u}\big)^2 \Big); \quad\quad \wt{\kappa} = \wt{D} / \lambda_{\min}(H).
	\end{equation*}
\end{proposition}

\begin{proof} \hspace{1mm} \\ \vspace{-5mm}
	
	\begin{enumerate}
		\item By definition of $\mathcal{M}_{\wt{D}}$, $\Tr\big(P(K_{\mu,\nu}) \big) \leq \wt{D}$ where $P(K_{\mu,\nu})$ is defined in Eq.~\ref{eq:average.cost.constraints.lyapunov2}. Thus, standard Lyapunov manipulation ensures that 
		\begin{equation*}
		\lambda_{\min}(H) \|A^c_{\mu,\nu}\|_F^2 \leq \Tr\big(P(K_{\mu,\nu}) \big) \leq \wt{D} \quad \Rightarrow \quad \|A^c_{\mu,\nu}\|_F \leq \sqrt{\wt{\kappa}}.
		\end{equation*}
		Let $\wt{\theta}^\transp = \begin{pmatrix} A & \wt{B} \end{pmatrix}= \begin{pmatrix} A & B & I \end{pmatrix}$ one has $A^c_{\mu,\nu} = \wt{\theta}^\transp \begin{pmatrix} I \\ K_{\mu,\nu}\end{pmatrix}$ and $\sigma_{\min}(\wt{\theta}) \geq 1$. Hence, 
		\begin{equation*}
		\left\|\begin{pmatrix} I \\ K_{\mu,\nu}\end{pmatrix}\right\|_F \leq \sigma_{\min}(\wt{\theta}) \left\|\begin{pmatrix} I \\ K_{\mu,\nu}\end{pmatrix}\right\|_F \leq \left\| \wt{\theta}^\transp \begin{pmatrix} I \\ K_{\mu,\nu}\end{pmatrix} \right\|_F = \|A^c_{\mu,\nu}\|_F \leq \sqrt{\wt{\kappa}} \quad \Rightarrow \quad \|K_{\mu,\nu}\|_F \leq \sqrt{\wt{\kappa}}.
		\end{equation*}
		
		
		\item For all $(\mu,\nu) \in \mathcal{M}_{\wt{D}}$, let $d_\mu P_{\mu,\nu}$ and $d_\nu P_{\mu,\nu}$ be the matrix derivatives w.r.t. to $\mu$ and $\nu$ respectively, as given in Eq.~\ref{eq:derivative.riccati.cost.matrix}. Then,
		\begin{equation*}
		\begin{aligned}
		- \frac{\|V^{-1}\|_2 \wt{\kappa}}{\lambda_{\min}(H) } P(K_{\mu,\nu}) \preccurlyeq d_\mu P_{\mu,\nu} \preccurlyeq \frac{\wt{\kappa}^2}{\lambda_{\min}(H)} P(K_{\mu,\nu}) \quad &\text{ and } \quad 0 \preccurlyeq d_\nu P_{\mu,\nu} \preccurlyeq \frac{1 + \|K_0\|_2^2}{\lambda_{\min}(H)} P(K_{\mu,\nu})
		\end{aligned}
		\end{equation*}
		As a result, we obtain the following bounds for the 2-norm:
		\begin{equation*}
		\|d_\mu P_{\mu,\nu}\|_2 \leq \kappa^2 \max(\kappa, \|V^{-1}\|_2) \quad \text{ and } \quad \|d_\nu P_{\mu,\nu}\|_2 \leq \wt{\kappa}\big(1 + \|K_0\|_2^2\big),
		\end{equation*}
		while taking the trace, we obtain the following bounds for the absolute values of the derivatives of $\mathcal{D}$:
		\begin{equation*}
		| \mathcal{D}^\prime_\mu(\mu,\nu)| \leq \kappa^2 \max\big(\kappa, \|V^{-1}\|_2 \big) \quad \text{ and } \quad |\mathcal{D}^\prime_\nu(\mu,\nu)| \leq \max\Big( \wt{\kappa}\big(1 + \|K_0\|_2^2\big), \big( \epsilon_0^{u}\big)^2 \Big).
		\end{equation*}
		
	\end{enumerate}
\end{proof}

\subsection{Step 2)} 
\begin{proposition}\label{p:lipschitz.riccati}
	
	The mapping $(\mu,\nu) \rightarrow P_{\mu,\nu}$ and $(\mu,\nu) \rightarrow \D_{\mu,\nu}$ are Lipschitz on $\mathcal{M}_{\wt{D}}$. Formally, for all $(\mu_1,\nu_1) \in \mathcal{M}_{\wt{D}}$ and $(\mu_2,\nu_2) \in \mathcal{M}_{\wt{D}}$, let $P_{\mu_1,\nu_1}$ and $P_{\mu_2,\nu_2}$ be the Riccati solutions, $\D(\mu_1,\nu_1)$ and $\D(\mu_2,\nu_2)$ the associated dual values, 
	\begin{equation*}
	\begin{aligned}
	\|P_{\mu_1,\nu_1} - P_{\mu_2,\nu_2}\|_2 &\leq l_\D \| (\mu_1,\nu_1) - (\mu_2,\nu_2)\|, \\
	|\D(\mu_1,\nu_1) - \D(\mu_2,\nu_2)| &\leq l_\D \| (\mu_1,\nu_1) - (\mu_2,\nu_2)\|,
	\end{aligned}
	\end{equation*}
	where $l_\D = \sqrt{l^2_\mu + l^2_\nu}$, $l_\mu$ and $l_\nu$ are given in Prop.~\ref{p:stable.bounded.set}.
\end{proposition}
\begin{proof}
	Exploiting the decomposition of the Riccati solution $P_{\mu,\nu} = P(K_{\mu,\nu}) + \mu d_\mu P_{\mu,\nu} + \nu d_\nu P_{\mu,\nu}$ and that $P_{\mu_1,\nu_1} \preccurlyeq P_{\mu_1,\nu_1}(K_{\mu_2,\nu_2})$, one obtains that
	\begin{equation*}
	P_{\mu_1,\nu_1} - P_{\mu_2,\nu_2} \preccurlyeq (\mu_1 - \mu_2) d_\mu P_{\mu_2,\nu_2} + (\nu_1 - \nu_2) d_\nu P_{\mu_2,\nu_2}.
	\end{equation*}
	Inverting the role of $(\mu_1,\nu_1)$ and $(\mu_2,\nu_2)$ we also get
	\begin{equation*}
	P_{\mu_2,\nu_2} - P_{\mu_1,\nu_1} \preccurlyeq (\mu_2 - \mu_1) d_\mu P_{\mu_1,\nu_1} + (\nu_2 - \nu_1) d_\nu P_{\mu_1,\nu_1}.
	\end{equation*}
	Finally, from Prop.~\ref{p:stable.bounded.set} we obtain that 
	\begin{equation*}
	\|P_{\mu_2,\nu_2} - P_{\mu_1,\nu_1} \|_2 \leq |\mu_2 - \mu_1| l_\mu + |\nu_2 - \nu_1| l_\nu.
	\end{equation*}
	A similar derivation for the trace of $P_{\mu,\nu}$ provides the Lipschitz continuity of $\mathcal{D}$.
\end{proof}

\begin{proposition}\label{p:lipschitz.control}
	The mapping $(\mu,\nu) \rightarrow K_{\mu,\nu}$ is Lipschitz on $\mathcal{M}_{\wt{D}}$. Formally, for all $(\mu_1,\nu_1) \in \mathcal{M}_{\wt{D}}$ and $(\mu_2,\nu_2) \in \mathcal{M}_{\wt{D}}$, let $K_{\mu_1,\nu_1}$ and $K_{\mu_2,\nu_2}$ be the optimal control, 
	\begin{equation*}
	\|K_{\mu_1,\nu_1} - K_{\mu_2,\nu_2}\| \leq l_K \| (\mu_1,\nu_1) - (\mu_2,\nu_2)\|,
	\end{equation*}
	where $l_K = \Big( \sqrt{2\wt{\kappa}} \max\big(1,\|V^{-1}\|_2 \big) + \sqrt{\wt{\kappa}} \|\wt{B}\|_2^2 l_\D + \|\wt{B}\|_2 \|A\|_2 l_\D + \sqrt{\| V^{-1}\|^2_2 +\| K_0\|^2_2} \Big) / \alpha$, $l_\D$ is given in Prop.~\ref{p:lipschitz.riccati} while $\alpha$ is given in Lem.~\ref{le:positivity.margin}.
\end{proposition}

\begin{proof}
	
	Let $D_{\mu_i,\nu_i} = R_{\mu_i,\nu_i} + \wt{B}^\transp P_{\mu_i,\nu_i} \wt{B}$ for all $i = 1,2$. By definition,
	\begin{equation*}
	\begin{aligned}
	& D_{\mu_2,\nu_2} K_{\mu_2,\nu_2} = - \big( \wt{B}^\transp P_{\mu_2,\nu_2} A + N_{\mu_2,\nu_2}\big) \quad \text{ and } \quad D_{\mu_1,\nu_1} K_{\mu_1,\nu_1} = - \big( \wt{B}^\transp P_{\mu_1,\nu_1} A + N_{\mu_1,\nu_1} \big) \\
	\Rightarrow & \quad D_{\mu_1,\nu_1} (K_{\mu_2,\nu_2} - K_{\mu_1,\nu_1}) = (D_{\mu_2,\nu_2} - D_{\mu_1,\nu_1} ) K_{\mu_2,\nu_2} + \wt{B}^\transp P_{\mu_1,\nu_1} A + N_{\mu_1,\nu_1} - \wt{B}^\transp P_{\mu_2,\nu_2} A + N_{\mu_2,\nu_2}.
	\end{aligned}
	\end{equation*}
	Further, 
	\begin{equation*}
	\begin{aligned}
	& \| (D_{\mu_2,\nu_2} - D_{\mu_1,\nu_1} ) K_{\mu_2,\nu_2} \|_2 \leq \| K_{\mu_2,\nu_2} \|_2 \big( \|R_{\mu_2,\nu_2} - R_{\mu_1,\nu_1}\|_2 + \|\wt{B}\|_2^2 \| P_{\mu_2,\nu_2} - P_{\mu_1,\nu_1} \|_2 \big), \\
	& \| \wt{B}^\transp P_{\mu_1,\nu_1} A + N_{\mu_1,\nu_1} - \wt{B}^\transp P_{\mu_2,\nu_2} A + N_{\mu_2,\nu_2} \|_2 \leq \|\wt{B}\|_2 \|A\|_2 \| P_{\mu_2,\nu_2} - P_{\mu_1,\nu_1} \|_2 + \|N_{\mu_2,\nu_2} - N_{\mu_1,\nu_1}\|_2.
	\end{aligned}
	\end{equation*}
	From Prop.~\ref{p:stable.bounded.set}, $\|K_{\mu_i,\nu_i}\|_2 \leq \sqrt{\wt{\kappa}}$, hence Lem.~\ref{le:positivity.margin} holds and $D_{\mu_i,\nu_i} \succcurlyeq \alpha I$. Moreover, 
	\begin{equation*}
	\begin{aligned}
	\|R_{\mu_2,\nu_2} - R_{\mu_1,\nu_1}\|_2 & \leq \sqrt{2} \max\big(1,\|V^{-1}\|_2 \big) \|(\mu_2,\nu_2) - (\mu_1,\nu_1)\|\\
	\|N_{\mu_2,\nu_2} - N_{\mu_1,\nu_1}\|_2 &\leq \sqrt{\| V^{-1}\|^2_2 +\| K_0\|^2_2} \|(\mu_2,\nu_2) - (\mu_1,\nu_1)\| \\
	\| P_{\mu_2,\nu_2} - P_{\mu_1,\nu_1} \|_2&\leq l_\D \|(\mu_2,\nu_2) - (\mu_1,\nu_1)\|
	\end{aligned}
	\end{equation*}
	Thus,
	\begin{equation*}
	\begin{aligned}
	\|D_{\mu_1,\nu_1} (K_{\mu_2,\nu_2} - K_{\mu_1,\nu_1})\|_2 &\leq \Big( \sqrt{2\wt{\kappa}} \max\big(1,\|V^{-1}\|_2 \big) + \sqrt{\wt{\kappa}} \|\wt{B}\|_2^2 l_\D + \|\wt{B}\|_2 \|A\|_2 l_\D + \sqrt{\| V^{-1}\|^2_2 +\| K_0\|^2_2} \Big) \|(\mu_2,\nu_2) - (\mu_1,\nu_1)\| \\
	\Rightarrow &\quad \|K_{\mu_2,\nu_2} - K_{\mu_1,\nu_1}\|_2 \leq l_K \|(\mu_2,\nu_2) - (\mu_1,\nu_1)\|,
	\end{aligned}
	\end{equation*}
	where $l_K = \Big( \sqrt{2\wt{\kappa}} \max\big(1,\|V^{-1}\|_2 \big) + \sqrt{\wt{\kappa}} \|\wt{B}\|_2^2 l_\D + \|\wt{B}\|_2 \|A\|_2 l_\D + \sqrt{\| V^{-1}\|^2_2 +\| K_0\|^2_2} \Big) / \alpha$.
\end{proof}


\subsection{Step 3)}
\begin{proposition}
	\label{p:constraint.continuity}
	The mapping $(\mu,\nu) \rightarrow \nabla \D (\mu,\nu)$ is Lipschitz on $\mathcal{M}_{\wt{D}}$. Formally, for all $(\mu_1,\nu_1) \in \mathcal{M}_{\wt{D}}$ and $(\mu_2,\nu_2) \in \mathcal{M}_{\wt{D}}$, one has:
	\begin{equation*}
	\begin{aligned}
	&| \mathcal{D}^\prime_\mu(\mu_1,\nu_1) - \mathcal{D}^\prime_\mu(\mu_2,\nu_2) | \leq 4 \sqrt{\wt{\kappa}} \|\wt{\theta}\|^2_2 l_\mu l_K \|(\mu_1,\nu_1) - (\mu_2,\nu_2)\| \\
	& | \mathcal{D}^\prime_\nu(\mu_1,\nu_1) - \mathcal{D}^\prime_\nu(\mu_2,\nu_2) | \leq 4 \sqrt{\wt{\kappa}} \|\wt{\theta}\|^2_2 l_\nu l_K \|(\mu_1,\nu_1) -(\mu_2,\nu_2)\|, \\
	& \| \nabla \D(\mu_1,\nu_1) - \nabla \D(\mu_2,\nu_2) \| \leq 4 \sqrt{\wt{\kappa}} \|\wt{\theta}\|^2_2 l_\D l_K \|(\mu_1,\nu_1) -(\mu_2,\nu_2)\|.
	\end{aligned}
	\end{equation*}
\end{proposition}

\begin{proof}
	The proof follows similar path for both inequalities, thus we only report a proof for the derivative w.r.t. $\mu$. Let $K_1 = K_{\mu_1,\nu_1}$, $K_2 = K_{\mu_2,\nu_2}$, $A_c^1 = A + \tilde{B} K_1$, $A_c^2 = A + \tilde{B} K_2$, $dP_1 = d_\mu P_{\mu_1,\nu_1}$ and $dP_{2} = d_\mu P_{\mu_2,\nu_2}$. Then, from 
	\begin{equation*}
	dP_1 = A_c^{1,\transp} dP_1 A_c^{1} + \begin{pmatrix} I \\ K_1 \end{pmatrix}^\transp C_g \begin{pmatrix} I \\ K_1 \end{pmatrix}; \quad \quad dP_2 = A_c^{2,\transp} dP_2 A_c^{2} + \begin{pmatrix} I \\ K_2 \end{pmatrix}^\transp C_g \begin{pmatrix} I \\ K_2 \end{pmatrix};
	\end{equation*}
	one gets $dP_1 - dP_2 = A_c^{1,\transp} dP_1 A_c^{1} + Z$ where
	\begin{equation*}
	2 Z = (A_c^2 - A_c^1)^\transp dP_2 (A_c^{2} + A_c^{1}) + (A_c^2 + A_c^1)^\transp dP_2 (A_c^{2} - A_c^{1}) + \begin{pmatrix} 2 I \\ K_1 + K_2\end{pmatrix}^\transp C_g \begin{pmatrix} I \\ K_1 - K_2 \end{pmatrix} + \begin{pmatrix} 0 \\ K_1 - K_2 \end{pmatrix}^\transp C_g \begin{pmatrix} 2I \\ K_1 + K_2 \end{pmatrix}.
	\end{equation*}
	Moreover, by Prop.~\ref{p:stable.bounded.set} and Prop.~\ref{p:lipschitz.control}, $\|K_1\|_2 \leq \sqrt{\wt{\kappa}}$, $\|K_2\|_2 \leq \sqrt{\wt{\kappa}}$, $\|dP_2\|_2 \leq l_\mu$ and $\|K_1 - K_2\|_2 \leq l_K \| (\mu_1,\nu_1) - (\mu_2,\nu_2)\|$. Thus,
	\begin{equation*}
	\begin{aligned}
	\|Z\|_2 &\leq 2 \sqrt{\wt{\kappa}}\|dP_2\|_2 \|\wt{\theta}\|_2 \| A_c^{1} - A_c^{2} \|_2 + 2\sqrt{\wt{\kappa}} \|C_g\|_2 \| K_1 - K_2\|_2 \\
	&\leq 2 \sqrt{\wt{\kappa}} \Big( \|\wt{\theta}\|^2_2 l_\mu + \max\big(1, \|V^{-1}\|_2 \big) \Big) \| K_1 - K_2\|_2 \\
	&\leq 2 \sqrt{\wt{\kappa}} \Big( \|\wt{\theta}\|^2_2 l_\mu + \max\big(1, \|V^{-1}\|_2\big) \Big) l_K \| (\mu_1,\nu_1) - (\mu_2,\nu_2)\|\\
	&\leq 4 \sqrt{\wt{\kappa}} \|\wt{\theta}\|^2_2 l_\mu l_K \| (\mu_1,\nu_1) - (\mu_2,\nu_2)\|\\
	\end{aligned}
	\end{equation*}
	Finally, we obtain $| \mathcal{D}^\prime_\mu(\mu_1,\nu_1) - \mathcal{D}^\prime_\mu(\mu_2,\nu_2) | = | \Tr(dP_1) - \Tr(dP_2)| \leq \|Z\|_2 \Tr(X) \leq \|Z\|_2 \tilde{D}$. Repeating the proof for $d_\nu P_{\mu,\nu}$ leads to the desired result.
	%\begin{equation*}
	%| \mathcal{D}^\prime_\mu(\mu_1,\nu_1) - \mathcal{D}^\prime_\mu(\mu_2,\nu_2) | = | \Tr(dP_1) - \Tr(dP_2)| \leq \|Z\|_2 \Tr(X) \leq \|Z\|_2 \tilde{D}, 
	%\end{equation*}
\end{proof}


\subsection{Proof of Cor.~\ref{co:smoothness.avg.cost.control}}

We proceed as in the proof of Prop.~\ref{p:constraint.continuity}. Let $K_1 = K_{\mu_1,\nu_1}$, $K_2 = K_{\mu_2,\nu_2}$, $A_c^1 = A + \tilde{B} K_1$, $A_c^2 = A + \tilde{B} K_2$, $P_1 = P(K_{\mu_1,\nu_1})$ and $P_{2} = P(K_{\mu_2,\nu_2})$. Then, from 
\begin{equation*}
P_1 = A_c^{1,\transp} P_1 A_c^{1} + \begin{pmatrix} I \\ K_1 \end{pmatrix}^\transp C_\dagger \begin{pmatrix} I \\ K_1 \end{pmatrix}; \quad \quad P_2 = A_c^{2,\transp} dP_2 A_c^{2} + \begin{pmatrix} I \\ K_2 \end{pmatrix}^\transp C_\dagger \begin{pmatrix} I \\ K_2 \end{pmatrix};
\end{equation*}
one gets $P_1 - P_2 = A_c^{1,\transp} P_1 A_c^{1} + Z$ where
\begin{equation*}
2 Z = (A_c^2 - A_c^1)^\transp P_2 (A_c^{2} + A_c^{1}) + (A_c^2 + A_c^1)^\transp P_2 (A_c^{2} - A_c^{1}) + \begin{pmatrix} 2 I \\ K_1 + K_2\end{pmatrix}^\transp C_\dagger \begin{pmatrix} I \\ K_1 - K_2 \end{pmatrix} + \begin{pmatrix} 0 \\ K_1 - K_2 \end{pmatrix}^\transp C_\dagger \begin{pmatrix} 2I \\ K_1 + K_2 \end{pmatrix}.
\end{equation*}
By construction $\|P_2\|_2 \leq \wt{D}$, $\|K_1\|_2 \leq \sqrt{\wt{\kappa}}$, $\|K_2\|_2 \leq \sqrt{\wt{\kappa}}$ and $\|C_\dagger\|_2 \leq \lambda_{max}(H)$. Thus,
\begin{equation*}
\begin{aligned}
\|Z\|_2 &\leq 2 \sqrt{\wt{\kappa}}\|P_2\|_2 \|\wt{\theta}\|_2 \| A_c^{1} - A_c^{2} \|_2 + 2\sqrt{\wt{\kappa}} \|C_\dagger\|_2 \| K_1 - K_2\|_2 \\
&\leq 2 \sqrt{\wt{\kappa}} \Big( \|\wt{\theta}\|^2_2 \wt{D} +\lambda_{\max}(H) \big) \Big) \| K_1 - K_2\|_2.
\end{aligned}
\end{equation*}







==> app_proof_duality_domain.tex <==
% !TEX root = main.tex

\subsubsection{Domain of Admissible Riccati Solutions}\label{ssec:app.dual.domain}

In the previous section we identified the condition for which at a specific Lagrangian parameter $\mu$, the solution of~\cref{eq:lagrangian.lqr.min} is obtained by solving a Riccati equation. We now proceed with characterizing the set of $\mathcal{M}$ in which \cref{eq:admissible.riccati.solution} holds.

%\paragraph{Admissible Riccati domain.}
Clearly, for $\{ \mu \in \Re^+ \text{ s.t } C_\mu \succ 0\}$,~\cref{eq:admissible.riccati.solution} holds as it coincides with the "standard" LQR setting. However, this set can be extended to a larger one, that we denote as $\mathcal{M}$.
We first relate the existence of a Riccati solution to a certain Popov criterion. Following~\citet{molinari1975}, we introduce the Popov functions:
\begin{definition}
\label{def:popov.function}
The Popov function $\Psi_{\mu}(\cdot,\sys)$ associated with $\sys \in \Sys$ and Lagrangian parameter $\mu$ is defined as:
\begin{equation}
\label{eq:popov.function.definition}
\Psi_{\mu}(z; \sys) = \begin{pmatrix} (I z^{-1} - A)^{-1} \tilde{B} \\ I \end{pmatrix}^\transp C_\mu \begin{pmatrix} (I z - A)^{-1} \tilde{B} \\ I \end{pmatrix}, \quad \forall z \in \mathbb{C}, \hspace{1mm} |z| = 1.
\end{equation}
For any controller $\wt{K}$, the controlled Popov function $\Psi_{\mu}^{\wt{K}}(\cdot,\sys)$ associated with $\sys \in \Sys$ and Lagrangian parameter $\mu$ is defined as:
\begin{equation}
\label{eq:popov.K.definition}
\Psi_{\mu}^{\wt K} (z)  = \begin{pmatrix} (I z^{-1} - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix}^\transp \begin{pmatrix} I & \wt{K}^\transp \\ 0 & I \end{pmatrix} C_\mu \begin{pmatrix} I & 0 \\ \wt K & I \end{pmatrix} \begin{pmatrix} (I z - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix}
\end{equation}
\end{definition}
In essence, the controlled Popov function by $\wt{K}$ simply consists in the Popov function when $\sys$ is pre-controlled by $\wt{K}$. The link between those two is given by
\begin{equation}
\label{eq:from.popov.controlled.popov}
\Psi_{\mu}^{\wt K} (z)  = Y^{\wt{K}}(z^{-1})^\transp \Psi_{\mu}(z) Y^{\wt{K}}(z)  \quad \quad \text{where} \quad Y^{\wt{K}}(z) = I + \wt K [Iz - \Ac(\wt K)]^{-1} \tilde{B}.
\end{equation}

The interest of considering Popov functions rather than solution of~\cref{eq:admissible.riccati.solution} is that the latter are well defined for all $\mu \geq 0$ while the former may not. Further, one can map the existence of a solution to~\cref{eq:admissible.riccati.solution} to the positive definiteness of the Popov functions. Those results are provided in~\citep{molinari1975}.
\begin{proposition}[Thm.1\&2~\citet{molinari1975}]\label{th:molinari75.1}
For any controllable system, the following conditions are equivalent:
\begin{enumerate}
	\item There exists a real symmetric solution satisfying Eq.~\eqref{eq:admissible.riccati.solution}, necessarily unique.
	\item For some (and hence all) $\wt K$ such that $|\lambda\big(\Ac_{\mu}(\wt{K})\big)| \neq 1$, $\Psi_{\mu}^{\wt K}(z) \succ 0$ on the unit circle $|z| = 1$.
\end{enumerate}
\end{proposition}
%
We also recall two important identities can be extracted from~\citet{molinari1975} that links the Popov function to the optimal quantities $\Ac_\mu$, $D_\mu$, $\wt{K}_\mu$ whenever they are defined:
\begin{equation}
\label{eq:popov.identities}
\begin{aligned}
&\forall |z| =1, \quad \Psi_{\mu}^{\wt K_\mu} (z) = D_\mu; &\\
& \forall |z| =1, \forall \wt{K} \text{ s.t } | \lambda(\Ac(\wt{K}))| \neq 1, & \Psi_{\mu}^{\wt K} (z)  =Y^{\wt{K},\wt{K}_{\mu}}(z^{-1})^\transp \Psi_{\mu}^{\wt K_\mu} (z)Y^{\wt{K},\wt{K}_{\mu}}(z), \\
&& \text{where} \quad Y^{\wt{K},\wt{K}_{\mu}}(z) = I + (\wt{K} - \wt{K}_{\mu}) [Iz - \Ac(\wt K)]^{-1} \tilde{B}.
\end{aligned}
\end{equation}
%
Thanks to~\cref{th:molinari75.1}, we can now associate to any $\sys \in \Sys$ a set $\mathcal{M}$ such that for all $\mu \in \mathcal{M}$, a symmetric solution to~\cref{eq:admissible.riccati.solution} exists and is strictly stabilizing, which, by~\cref{le:riccati.lqr.solution} implies that the optimal solution to~\cref{eq:lagrangian.lqr.min} is a linear policy.
\begin{lemma}\label{prop:domain.mutilde.nu}
For any $\sys \in \Sys$, let $\Psi_{\mu}^{\wt K}(z,\sys)$ be defined by~\cref{def:popov.function}. Let
\begin{equation}\label{eq:mutilde.definition}
\tilde{\mu} := \sup \big\{ \mu \geq 0 \text{ s.t. }\; \Psi_{\mu}^{\wt K}(z) \succ 0,\; \text{ for all } |z| = 1 \text{ and } \wt K \text{ such that } |\lambda\big(\Ac_{\mu}(\wt{K})\big)| \neq 1\big\}.
\end{equation}
Then, the set $\mathcal{M} = [0, \wt{\mu})$ is non-empty and for all $\mu \in\M$, Eq.~\eqref{eq:admissible.riccati.solution} admits a solution such that $\rho(\Ac_{\mu}) < 1$.
\end{lemma}

\begin{proof} 
\begin{enumerate}
\item For $\mu = 0$, 
\begin{equation*}
C_0 = C_\dagger + 0  \times C_g =  \begin{pmatrix} C_\dagger^1 & 0 \\ 0 & 0 \end{pmatrix} + C_\dagger^2.
\end{equation*}
From $C_\dagger^1 \succ 0$ and $C_\dagger^2 \succcurlyeq 0$, one has for all $\wt K$ such that $|\lambda\big(\Ac_{\mu}(\wt{K})\big)| \neq 1$, for all $|z|=1$,
\begin{equation*}
\begin{aligned}
\Psi_{0}^{\wt K}(z)  &= \begin{pmatrix} (I z^{-1} - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix}^\transp \begin{pmatrix} I & \wt{K}^\transp \\ 0 & I \end{pmatrix} C_\dagger \begin{pmatrix} I & 0 \\ \wt K & I \end{pmatrix} \begin{pmatrix} (I z - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix} \\
&\succcurlyeq  \begin{pmatrix} (I z^{-1} - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix}^\transp \begin{pmatrix} I & \wt{K}^\transp \\ 0 & I \end{pmatrix} \begin{pmatrix} C_\dagger^1 & 0 \\ 0 & 0 \end{pmatrix}  \begin{pmatrix} I & 0 \\ \wt K & I \end{pmatrix} \begin{pmatrix} (I z - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix} \\
&\succcurlyeq \begin{pmatrix} (I z^{-1} - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix}^\transp  \begin{pmatrix} I & \wt{K}^\transp \\ 0 & I \end{pmatrix}  \begin{pmatrix} I_{n+d} \\0 \end{pmatrix} C_\dagger^1 \begin{pmatrix} I_{n+d} & 0\end{pmatrix} \begin{pmatrix} I & 0 \\ \wt K & I \end{pmatrix} \begin{pmatrix} (I z - \Ac(\wt K))^{-1} \tilde{B} \\ I \end{pmatrix} \\
&\succ 0.
\end{aligned}
\end{equation*}
As a result, for all  $0 \in \mathcal{M}$ and $\mathcal{M}$ is non-empty.
 \item To show that all $\mu \in \mathcal{M}$ are associated with a strictly stabilizing solution of~\cref{eq:admissible.riccati.solution}, we invoque~\cref{th:molinari75.1}. As a result, we are left to prove that for all $\mu \in \mathcal{M}$, it exists $\wt{K}$ such that $|\lambda\big(\Ac_{\mu}(\wt{K})\big)| \neq 1$ and $\Psi^{\wt{K}}_{\mu}(z) \succ 0$ for all $|z|=1$.\\
 Exploiting the linearity of $\Psi_{\mu}$ (as $C_{\mu}$ is linear in $\mu$, for all $|z| =1$ and $\wt K$), so is $\Psi_{\mu}^{\wt K}(z)$. Hence, for all $|z|=1$, for all $v \in \mathbb{C}^{n+d} \setminus \{0\}$, the function 
 \begin{equation*}
 f : \mu \rightarrow v^* \Psi^{\wt{K}}_{\mu}(z) v,
 \end{equation*}
 is linear in $\mu$. Moreover, $\lim_{\mu \rightarrow \wt{\mu}} f(\mu) \geq 0$ and $f(0) > 0$, which implies that for all $\mu \in \mathcal{M}$, for all $|z|=1$,
 \begin{equation*}
 \forall v \in \mathbb{C}^{n+d}\setminus \{0\}, \quad  v^* \Psi^{\wt{K}}_{\mu}(z) v > 0 \quad \Rightarrow \quad \Psi^{\wt{K}}_{\mu}(z) \succ 0.
 \end{equation*}
\end{enumerate}
\end{proof}

\subsubsection{Characterization of $\mathcal{D}(\mu,\sys)$}\label{ssec:app.dual.characterization}

We are now ready to characterize the dual function $\mathcal{D}$. For any $\sys \in \Sys$, the use of the Popov functions allows us to define a set $\mathcal{M}$ (~\cref{prop:domain.mutilde.nu}) that depends explicitely (yet in a non-trivial fashion) in $\sys$, and on which the inner minimization problem~\cref{eq:lagrangian.lqr.min} corresponds to a well-defined (yet non-standard) Riccati equation. We summarize~\cref{le:riccati.lqr.solution,prop:domain.mutilde.nu} in~\cref{prop:dual.riccati} which proves the first statements of~\cref{lem:dual.function}.

\begin{proposition}
\label{prop:dual.riccati}
For any $\sys \in \Sys$, let $\mathcal{M}$ be the admissible Riccati set associated with $\sys$ as defined in~\cref{eq:mutilde.definition} and $\mathcal{D}(\mu,\sys)$ the dual function defined in~\cref{eq:lagrangian.lqr.min}. Then, \begin{enumerate}
\item for all $\mu \in \mathcal{M}$, it exists a unique symmetric matrix $P_\mu$ satisfying~\cref{eq:admissible.riccati.solution}, 
\item the optimal policy $\tpi_\mu(\cdot,\sys) = \arg\min_{\tpi}\mathcal L_{\tpi}(\mu ; \sys)$ is linear in the state, i.e., $\tpi_\mu(x,\sys)= \wt{K}_\mu x$, where 
\begin{equation*}
\wt K_{\mu} = - [ R_{\mu} + \tilde{B}^\transp P_{\mu} \tilde{B} ]^{-1} [ \tilde{B}^\transp P_{\mu} A + N_{\mu} ],
\end{equation*}
\item $\mathcal{J}_{\tpi_{\mu}}(\sys) = \Tr\big( P(\wt K_{\mu})\big)$, $g_{\tpi_{\mu}}(\sys) = \Tr\big(G(\wt K_{\mu})\big)$, $\mathcal{D}(\mu,\sys) = \mathcal{L}_{\tpi_{\mu}}(\mu,\sys) = \Tr\big( P_\mu\big)$.
\item $\mu  \rightarrow \mathcal{D}(\mu,\sys)$ is concave on $\mathcal{M}$ and $\mathcal{D}(\mu, \sys) > - \infty$ on $\mathcal{M}$.
\item $\mu  \rightarrow \mathcal{D}(\mu,\sys) \in \mathcal{C}^{1}(\mathcal{M})$.
\end{enumerate}
\end{proposition}

\begin{proof}
The proof of~\cref{prop:dual.riccati} directly follows from merging~\cref{le:riccati.lqr.solution} and~\cref{prop:domain.mutilde.nu}.
\end{proof}

Now that~\cref{prop:dual.riccati} guarantees that for any $\sys\in\Sys$, $\mathcal{D}(\cdot,\sys)$ is well defined on some explicit convex set $\mathcal{M}$, we are able to prove the last statements of~\cref{lem:dual.function}.
\begin{proposition}
\label{prop:derivative.riccati.cost.matrix}
For any $\sys \in \Sys$, let $\mathcal{M}$ be the admissible Riccati set associated with $\sys$ as defined in~\cref{eq:mutilde.definition}. Let $\mathcal{D}^\prime$ denote the derivative of $\mathcal{D}$ w.r.t. $\mu$. Then,
\begin{enumerate}
\item $\mathcal{M}$ is a non-empty convex set,
\item $\mu  \rightarrow \mathcal{D}(\mu,\sys)$ is concave on $\mathcal{M}$ and $\mathcal{D}(\mu, \sys) > - \infty$ on $\mathcal{M}$.
\item $\mu  \rightarrow \mathcal{D}(\mu,\sys) \in \mathcal{C}^{1}(\mathcal{M})$.
\item $\D^\prime(\mu,\sys)) =g_{\tpi_\mu}(\sys) = \Tr(G(\wt{K}_\mu))$, where $\wt{K}_\mu$ and $\wt\pi_{\mu}(x) = \wt K_{\mu} x$ be respectively the optimal controller and policy as defined in~\cref{prop:dual.riccati} and $G(\wt{K}_\mu)$ is given in~\cref{eq:average.cost.constraints.lyapunov2}. As a result,
\begin{equation}
\label{eq:lagrangian.dual.derivative}
\mathcal{D}(\mu,\sys) = \mathcal{J}_{\tpi_{\mu}}(\sys) + \mu g_{\tpi_{\mu}}(\sys) = \mathcal{J}_{\tpi_{\mu}}(\sys) + \mu \mathcal{D}^\prime(\mu,\sys).
\end{equation}
\end{enumerate}
\end{proposition}


\begin{proof}
\begin{enumerate}
\item $\mathcal{M}$ is non-empty from~\cref{prop:domain.mutilde.nu}. Further, $\mathcal{M} = [0,\wt{\mu})$ where $\wt{\mu}$ is defined in~\cref{eq:mutilde.definition}. Thus, $\mathcal{M}$ is convex.
\item The concavity of $\mathcal{D}(\cdot,\sys)$ is provided by construction, as $\mathcal{D}$ is the minimum of affine function. The lower boundedness property of $\mathcal{D}(\cdot,\sys)$ follows from $D_\mu  = R_\mu + \wt{B}^\transp P_\mu \wt{B} \succ 0$ for all $\mu \in \mathcal{M}$. Since $\R_\mu \prec +\infty$ and $\wt{B}$ is full column rank, 
\begin{equation*}
\D_\mu \succ 0 \quad \Rightarrow  \quad \wt{B}^\transp P_\mu \wt{B} \succ -\infty \quad \Rightarrow \quad P_\mu \succ - \infty \quad \Rightarrow \quad  \D(\mu,\sys) = \Tr(P_\mu) > - \infty.
\end{equation*}
\item The smoothness of $\mathcal{D}(\cdot,\sys)$ follows from Alexandrov's Theorem that guarantees that $\mathcal{D}(\cdot,\sys)$ is twice differentiable on $\mathcal{M}$ and hence in $\mathcal{C}^{1}(\mathcal{M})$.
\item $g_{\tpi_\mu}(\sys) = \Tr(G(\wt{K}_\mu))$ by~\cref{prop:dual.riccati}. We are thus left to prove that $\D^\prime(\mu,\sys)) =g_{\tpi_\mu}(\sys)$, which is a structural property inherited from the Lagrangian formulation and that is directly implied by the fact that $\mathcal{D}(\mu,\sys) > \infty$ for all $\mu \in \mathcal{M}$ and that $\mathcal{D}(\cdot,\sys)$ is smooth and concave. Observe that by construction, for any $(\mu,\wb{\mu}) \in \mathcal{M}^2$, 
\begin{equation*}
\mathcal{D}(\wb{\mu},\sys) = \mathcal{J}_{\tpi_{\wb{\mu}}}(\sys) + \wb{\mu} g_{\tpi_{\wb{\mu}}}(\sys) = \min_{\tpi}\left(\mathcal{J}_{\tpi}(\sys) + \wb{\mu} g_{\tpi}(\sys) \right) \geq  \mathcal{J}_{\tpi_{\mu}}(\sys) + \wb{\mu} g_{\tpi_{\mu}}(\sys)  = \mathcal{D}(\mu,\sys) + (\wb{\mu} - \mu)g_{\tpi_{\mu}}(\sys).
\end{equation*}
Thus, $\mathcal{D}(\wb{\mu},\sys)  \geq \mathcal{D}(\mu,\sys) + (\wb{\mu} - \mu)g_{\tpi_{\mu}}(\sys)$ 
%\begin{equation}
%\label{eq:supergradient.concave.dual}
%\mathcal{D}(\wb{\mu},\sys)  \geq \mathcal{D}(\mu,\sys) + (\wb{\mu} - \mu)g_{\tpi_{\wb{\mu}}}(\sys),
%\end{equation}
which means by definition that $g_{\tpi_{\mu}}(\sys)$ belongs to the super-gradient set at $\mu$ (which is defined for concave function that are not $-\infty$, see~\citep{rockafellar1970convex} for a survey). However, since $\mathcal{D}(\cdot,\sys) \in \mathcal{C}^1(\mathcal{M}$, the super-gradient set is reduced to a singleton, which coincides with the derivative. As a result, $\mathcal{D}^\prime(\mu,\sys) = g_{\tpi_{\mu}}(\sys)$.
\end{enumerate}
\end{proof}







==> app_proof_duality_old.tex <==
% !TEX root = main.tex

\section{Proof of Thm.~\ref{thm:dual.gap}}\label{sec:app.proof.duality}
In this section, we consider here without loss of generality that $\beta = 1$ (otherwise, we just need to redefined $V^{-1} \leftarrow \beta^2 V^{-1}$). Further, we consider $\theta^\transp = [A,B] \in \mathbb{R}^{n\times (n+d)}$ such that $B$ is full column rank and $A - B V_{22} V_{21}^{-1}$ is full rank. Since those quantities are fixed during the whole analysis, we will drop the dependencies in $\mathcal{J}$, $g_{\pi}$ and $\mathcal{D}$. Finally, we recall that $\wt{B} = [B , I] \in \mathbb{R}^{n \times (d+n)}$ and that the extended pair $(A,\wt{B})$ is controllable even if the original one $(A,B)$ is not.\footnote{This can be easily shown as the extended controller $K^\transp = \begin{pmatrix} 0 & -A^\transp \end{pmatrix}$ induces a closed-loop matrix $A + \wt{B} K = 0$ and hence stable.}

The proof of Thm.~\ref{thm:dual.gap} heavily relies on the intermediate results used in proving Lemma~\ref{lem:dual.function} and Prop.~\ref{p:function.D}. We start by proving each sub-point of the lemma and the proposition and we finally derive the statement of the theorem. Lemma.~\ref{lem:dual.function} provides guarantees on the minimization and maximization problems
\begin{equation*}
\wt\pi_{\mu,\nu} = \arg\min_{\tpi}\mathcal L_{\tpi}(\mu,\nu) \quad \text{ and } \quad \sup_{\mu \in \Re_+} \mathcal{D}(\mu,\nu).
\end{equation*}
From Eq.~\ref{eq:lagrange.lqr}
\begin{equation}
\label{eq:extended.lqr.definition.mu.nu}
\begin{aligned}
\mathcal L_{\tpi}(\mu, \nu) &=\lim_{S \rightarrow \infty} \frac{1}{S} \mathbb{E} \bigg[ \sum_{s=0}^{S-1} \begin{pmatrix} x_s^\transp & \tilde{u}_s^\transp \end{pmatrix} H_{\mu,\nu} \begin{pmatrix} x_s \\ \tilde{u}_s \end{pmatrix} \bigg] - \nu(\epsilon_0^u)^2 \\
\text{subject to } &x_{s+1} = A x_s + \wt{B} \wt{u}_s+ \epsilon_{s+1}
\end{aligned}
\end{equation}
where 
\begin{equation*}
H^\dagger = \begin{pmatrix} Q & 0 & 0 \\ 0 & R & 0 \\ 0 & 0 & 0 \end{pmatrix}; \quad H_\mu = \mu \begin{pmatrix} - V^{-1} & 0 \\ 0 & I \end{pmatrix}; \quad H_\nu =\nu \begin{pmatrix} K_0^\transp K_0 & -K_0^\transp & 0 \\ -K_0 & I & 0 \\ 0 & 0 & 0 \end{pmatrix}
\end{equation*}

We conveniently rewrite the cost matrix $H_{\mu,\nu} = H^\dagger + H_\mu + H_\nu$ in a more standard form as 
\begin{equation}
\label{eq:cost.matrices.def.mu.nu}
\begin{aligned}
&H_{\mu,\nu} = \begin{pmatrix} Q_{\mu,\nu} & N_{\mu,\nu}^\transp  \\ N_{\mu,\nu} & R_{\mu,\nu} \end{pmatrix} \quad \text{ where } \quad Q_{\mu,\nu} := Q  - \mu V_{11}^{-1} + \nu K_0^\transp K_0;\\
 &N_{\mu,\nu} := \begin{pmatrix} - \mu V_{21}^{-1} - \nu K_0 \\ 0 \end{pmatrix}; \quad R_{\mu,\nu} := \begin{pmatrix} R - \mu V_{22}^{-1} + \nu I& 0 \\ 0 & \mu I \end{pmatrix}.
\end{aligned}
\end{equation}
From Eq.~\ref{eq:cost.matrices.def.mu.nu}, it is clear that minimizing $\mathcal L_{\tpi}(\mu, \nu)$ resembles solving an LQR problem. However, while for small (resp large) enough $\mu$  (resp $\nu$) values, the cost matrix $H_{\mu,\nu}$ is p.s.d. and the minimization coincides with a standard LQR, it is no longer the case as $\mu$ gets large since it breaks the positiveness of $H_{\mu,\nu}$. The proof of Lemma~\ref{lem:dual.function} is therefore split in three parts. First, we specify the domain of $(\mu,\nu)$ over which the minimization of $\mathcal L_{\tpi}(\mu, \nu)$ correspond to a non-standard yet well-defined LQR problem (Lemma~\ref{lem:dual.function}.1). Then, we characterize further the dual function $\mathcal{D}$ over this domain (Prop.~\ref{p:function.D}). Finally, we show that the dual maximization problem admits a solution within the domain (Lemma~\ref{lem:dual.function}.2).

\newpage
\subsection{Proof of Lemma~\ref{lem:dual.function}.1}\label{ssec:app.proof.extended.riccati1}
As hinted in the previous subsection, the extended LQR in~\eqref{eq:extended.lqr.definition.mu.nu} can be solved using standard Riccati equation whenever $\mu$ is small enough such that $H_{\mu,\nu}$ is p.s.d.\ Nonetheless, Riccati theory extends to a more general setting. Formally, we are interested in the existence of symmetric real matrices $P_{\mu,\nu}$ which satisfies the set of conditions:%\todoaout{$Q_\mu$ $R_\mu$, $N_\mu$ are not defined.}
\begin{equation}
\label{eq:admissible.riccati.solution}
\begin{aligned}
& R_{\mu,\nu}+ \tilde{B}^\transp P_{\mu,\nu} \tilde{B} \succ 0 \\
& P_{\mu,\nu} = Q_{\mu,\nu} + A^\transp P_{\mu,\nu} A  - [ A^\transp P_{\mu,\nu} \tilde{B} + N_{\mu,\nu}^\transp ] [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1} [ \tilde{B}^\transp P_{\mu,\nu} A + N_{\mu,\nu} ] \\
& | \lambda(A^c_{\mu,\nu}) | \leq 1 \quad \text{ where } \quad A^c_{\mu,\nu} := A - \tilde{B} [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1} [ \tilde{B}^\transp P_{\mu,\nu} A + N_{\mu,\nu} ].
\end{aligned}
\end{equation} 

The following Lemma maps the existence and uniqueness of a solution satisfying Eq.~\eqref{eq:admissible.riccati.solution} and the solution of the extended LQR.

\begin{lemma}
\label{le:riccati.lqr.solution}
If there exists a symmetric matrix $P_{\mu,\nu}$ satisfying Eq.~\eqref{eq:admissible.riccati.solution}, then
\begin{enumerate}
\item it is unique
\item it is the solution of the associated extended LQR problem, that is, $\mathcal{D}(\mu,\nu) = \Tr (P_{\mu,\nu})$ and $\wt\pi_{\mu,\nu}(x) = K_{\mu,\nu} x$ for all $x \in \mathbb{R}^n$ where $K_{\mu,\nu} = - [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1} [ \tilde{B}^\transp P_{\mu,\nu} A + N_{\mu,\nu} ]$.
\item for all matrix $K$, $P_{\mu,\nu} \preccurlyeq P_{\mu,\nu}(K)$ where $P_{\mu,\nu}(K) = A(K)^\transp P_{\mu,\nu}(K)A(K) + Q_{\mu,\nu}(K)$, with $A(K)$ and $Q(K)$ are defined as in Eq.~\ref{eq:controlled.matrix.def}
\end{enumerate}
\end{lemma}
Lem.~\ref{le:riccati.lqr.solution} directy follows from [Molinari, 1975, Thm.1] which ensures that if a solution to the Riccati equation exists, then it is unique. Further, it satisfies the Bellman equation, which ensures that $\mathcal{D}(\mu,\nu) = \Tr (P_{\mu,\nu})$ and that $\pi_{\mu,\nu}(x) = K_{\mu,\nu} x$ for all $x \in \mathbb{R}^n$ (see [Bertsekas, Vol.2, Prop.5.6.1]). Finally, the third assertion comes from the fact that for any control $K$, $\Delta =P_{\mu,\nu}(K) -  P_{\mu,\nu}$ statisfies the Lyapunov equation
\begin{equation}\label{eq:lyap.suboptimal.K}
\Delta = A_c(K)^\transp \Delta A_c(K) + (K_{\mu,\nu} - K)^\transp [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ] (K_{\mu,\nu} - K).
\end{equation}
Eq.~\ref{eq:lyap.suboptimal.K} directly implies that $P_{\mu,\nu} \preccurlyeq P_{\mu,\nu}(K)$ provided that $[R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ] \succ 0$. This highlights the role of this quantity, which controls the uniqueness of the optimal controller. Indeed, when $R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B}$ is arbitrarily close to $0$, it exists controllers $K \neq K_{\mu,\nu}$ with arbitrarily close value $P(K) \approx P_{\mu,\nu}$.\\

From Lem.~\ref{le:riccati.lqr.solution}, we can directly focus on Eq.~\ref{eq:admissible.riccati.solution} in order to prove the Lemma~\ref{lem:dual.function}.1. Now we need to display a domain for $(\mu,\nu)$ over which Lemma~\ref{le:riccati.lqr.solution} applies.

\paragraph{Popov criterion.}
The proof relies on the existence of a Riccati solution, which can be provided given that a certain \textbf{Popov criterion} is satisfied. Formally, we introduce the Popov function $\Psi_{\mu,\nu}(z)$ associated with the problem parametrized by $(A,\tilde{B},Q_{\mu,\nu}, N_{\mu,\nu}, R_{\mu,\nu})$ as:
\begin{equation}
\label{eq:popov.function.definition}
\Psi_{\mu,\nu}(z) = \begin{pmatrix} (I z^{-1} - A)^{-1} \tilde{B} \\ I \end{pmatrix}^\transp \begin{pmatrix} Q_{\mu,\nu} & N_{\mu,\nu}^\transp \\ N_{\mu,\nu} & R_{\mu,\nu} \end{pmatrix}  \begin{pmatrix} (I z - A)^{-1} \tilde{B} \\ I \end{pmatrix}, \quad \forall z \in \mathbb{C}, \hspace{1mm} |z| = 1.
\end{equation}
Additionally, for any control matrix $K$, we denote as $\Psi_{\mu,\nu}^{K} (z)$ the Popov function associated with the problem parametrized by $(A(K),\tilde{B},Q_{\mu,\nu}(K), N_{\mu,\nu}(K), R_{\mu,\nu})$ where 
\begin{equation}
\label{eq:controlled.matrix.def}
A(K) = A + \wt{B} K, \quad Q_{\mu,\nu}(K) = Q_{\mu,\nu} + N_{\mu,\nu}^\transp K + K^\transp N_{\mu,\nu} + K^\transp R_{\mu,\nu} K, \quad N_{\mu,\nu}(K) = N_{\mu,\nu} + R_{\mu,\nu} K.
\end{equation}
Standard algebraic manipulation shows easily that
\begin{equation}
\label{eq:popov.K.definition}
\Psi_{\mu,\nu}^{K} (z) = Y(z^{-1})^\transp \Psi_{\mu,\nu}(z)  Y(z), \quad \text{where} \quad Y(z) = I - K [Iz - A(K)]^{-1} \tilde{B}.
\end{equation}
Finally, from [Molinari, 1975], we have the two following important results:
\begin{theorem}[From Molinari, 1975, Thm.1]\label{th:molinari75.1}
	Let $(A,\tilde{B})$ be controllable. Then, the following conditions are equivalent:
	\begin{enumerate}
		\item There exists a real symmetric solution satisfying Eq.~\eqref{eq:admissible.riccati.solution}, necessarily unique.
		\item For some (and hence all) $K$, $\Psi_{\mu,\nu}^K(z) \succ 0$ on the unit circle $|z| = 1$, except perhaps on a finite number of point.
	\end{enumerate}
\end{theorem}

\begin{theorem}[From Molinari, 1975, Thm.2]\label{th:molinari75.2}
	Let $(A,\tilde{B})$ be controllable. Then, the following conditions are equivalent:
	\begin{enumerate}
		\item There exists a real symmetric solution satisfying Eq.~\eqref{eq:admissible.riccati.solution}, necessarily unique, and $|\lambda(A^c_{\mu,\nu})| < 1$.
		\item For some (and hence all) $K$ such that $|\lambda(A(K))| \neq 1$,  $\Psi_{\mu,\nu}^K(z) \succ 0$ for all $|z| = 1$.
	\end{enumerate}
\end{theorem}

\paragraph{Admissible Riccati domain.}
We are now ready to introduce a domain for $\mathcal{M} \subset \mathbb{R}_+^{2}$ such that for any $(\mu,\nu) \in \mathcal{M}$, Thm.~\ref{th:molinari75.2} holds. First, notice that by construction, for any $\nu \geq 0$ it exists a $K$ such that for all $\mu \in [0,\mu^+_{\nu})$, $\Psi_{\mu,\nu}^K(z) \succ 0$ where $$\mu^+_\nu = \sup \{\mu \geq 0 \text{ s.t. } H_{\mu,\nu} \succcurlyeq 0\} > 0.$$ Moreover, since $H_{\mu,\nu}$ is linear in $\mu$, for all $|z| =1$ and $K$, so is $\Psi_{\mu,\nu}^K(z)$. As a result, for any $\nu \geq 0$, there exists $\tilde{\mu}_\nu > 0$ defined as
\begin{equation}
\label{eq:mutilde.definition}
\tilde{\mu}_\nu := \min \{ \mu \geq 0 \text{ s.t. } \det \Psi_{\mu,\nu}^K(z) = 0 \text{ for some } |z| = 1 \text{ and } K\}.
\end{equation}
Further, we introduce a domain $\mathcal{M}$ as:
\begin{definition}
\label{def:riccati.domain}
$\mathcal{M} = \Big\{ (\mu,\nu) \in \mathbb{R}^2_+ \text{ such that } \mu < \wt{\mu}_\nu \text{ where } \wt{\mu}_{\nu} \text{ is defined as in Eq.~\ref{eq:mutilde.definition}} \Big\}.$
\end{definition}

This definition directly implies the following property:
\begin{property}\label{prop:domain.mutilde.nu}
$(\mu,\nu) \in \mathcal{M}$ if and only if  for all $K$, for all $|z|=1$, $\Psi_{\mu,\nu}^K(z) \succ 0$. Further, $\mathcal{M}$ is a convex set and $\nu \rightarrow \wt{\mu}_\nu$ is increasing.
\end{property}
\begin{proof}
We prove the first assertion by contradiction. Let $\nu \geq 0$ and $\mu \in [0, \tilde{\mu}_\nu)$, and assume that there exist some $K$ and $|z|=1$ such that $\Psi_{\mu,\nu}^K(z)$ is not positive definite (by definition it can only happen when $\mu \geq \mu_+ >0 $). Since $\Psi_{\mu,\nu}^K(z)$ is an hermitian matrix, it implies that $\lambda_{\min}(\Psi_{\mu,\nu}^K(z)) \leq 0$ and thus by continuity, it exists $\mu_0 \in [0,\mu]$ such that $\lambda_{\min}(\Psi^{\mu_0}_K(z)) = 0$. This implies that $\tilde{\mu}_\nu \leq \mu_0 \leq \mu$ and lead to the contradiction.\\
Controversy, since for all $K$ and all $|z|=1$, $\Psi_{0,\nu}^K(z) \succ 0$, by continuity $\Psi_{\mu,\nu}^K(z) \succ 0$ implies that $\det \Psi_{\wb{\mu},\nu}^K(z) > 0$ for all $\wb{\mu} \in [0,\mu]$ and hence that $\mu < \wt{\mu}_\nu$ i.e., $(\mu,\nu) \in \mathcal{M}$.\\

The convexity of $\mathcal{M}$ directly comes from the linearity of $\Psi_{\mu,\nu}$. Formally, for any pairs $(\mu_1,\nu_1) \in \mathcal{M}$ and $(\mu_2,\nu_2) \in \mathcal{M}$, given the first statement of Property.~\ref{prop:domain.mutilde.nu}, we just need to show that 
 $\Psi_{t\mu_1 + (1-t)\mu_2,t \nu_1 + (1-t) \nu_2}^K(z) \succ 0$ for all $t \in (0,1)$ for all $K$ and all $|z|=1$. Since for all $K$ and all $|z|=1$, $$\Psi_{t\mu_1 + (1-t)\mu_2,t \nu_1 + (1-t) \nu_2}^K(z) = t  \Psi_{\mu_1,\nu_1}^K(z)  + (1-t) \Psi_{\mu_2,\nu_2}^K(z)$$
one obtains the convexity of $\mathcal{M}$. Finally, the increasing property of the mapping $\nu \rightarrow \wt{\mu}_\nu$ follows from a similar reasoning, noting that for any $(\mu,\nu) \in \mathcal{M}$, for any $\bar{\nu} \geq \nu$, for all $K$ and all $|z|=1$, 
$$\Psi_{\mu,\bar{\nu}}^K(z) = \Psi_{\mu,\nu}^K(z)  + Y(z^{-1})^\transp \begin{pmatrix} (I z^{-1} - A)^{-1} \tilde{B} \\ I \end{pmatrix}^\transp \Big(H_{\bar{\nu}} - H_{\nu} \Big)\begin{pmatrix} (I z - A)^{-1} \tilde{B} \\ I \end{pmatrix}  Y(z) \succcurlyeq \Psi_{\mu,\nu}^K(z) $$
since $H_{\bar{\nu}} - H_{\nu} \succcurlyeq 0$.
\end{proof}
Using Thm.~\ref{th:molinari75.2}, this directly translates into 
\begin{property}\label{prop:domain.mutilde.2}
For all $(\mu,\nu) \in \mathcal{M}$, it exists a (necessarily unique) real symmetric solution $P_{\mu,\nu}$ satisfying Eq.~\eqref{eq:admissible.riccati.solution}, and $|\lambda(A^c_{\mu,\nu})| < 1$.
\end{property}
According to Lem.~\ref{le:riccati.lqr.solution}, this guarantees that for all $(\mu,\nu) \in \mathcal{M}$, \textbf{1)} $\mathcal{D}(\mu,\nu) = \Tr (P_{\mu,\nu})$, \textbf{2)} $\pi_{\mu,\nu}(x) = K_{\mu,\nu} x$ and is unique, which proves the first assertion in Lem.~\ref{lem:dual.function}.

\paragraph{Closure of $\mathcal{M}$.} Property.~\ref{prop:domain.mutilde.2} guarantees that the domain $\mathcal{M}$ coincides with the admissible Riccati domain, in the sense of Thm.~\ref{th:molinari75.2}. However, in order to prove Lemma~\ref{lem:dual.function}.2, we need to investigate the solution of Eq.~\ref{eq:admissible.riccati.solution} on the closure of $\mathcal{M}$, denoted as $\wb{\mathcal{M}}$, that is when $\mu \rightarrow \wt{\mu}_{\nu}$ for any $\nu \geq 0$. While in general $P_{\mu,\nu}$ may not be defined on the frontier of $\mathcal{M}$, the following Lemma states that $\wb{\mathcal{M}}$ coincides with an admissible Riccati domain in the sense of Thm.~\ref{th:molinari75.1}, provided that $A - B V_{22} V_{21}^{-1}$ is full rank and $B$ is full column rank.

\begin{lemma}\label{le:existence.closure.M}
Let $A - B V_{22} V_{21}^{-1}$ and $B$ be full (column) rank. Then, for all $(\mu,\nu) \in \wb{\mathcal{M}}$,
for some (and hence all) $K$, $\Psi_{\mu,\nu}^K(z) \succ 0$ on the unit circle $|z| = 1$ except on a finite number of points. As a result, it exists a symmetric matrix $P_{\mu,\nu}$ satisfying Eq.~\eqref{eq:admissible.riccati.solution}.
\end{lemma}
Interplaying with Prop.~\ref{prop:domain.mutilde.2} and Lem.~\ref{le:existence.closure.M}, we obtain a characterization of $A^c_{\mu,\nu}$ when $\mu \rightarrow \wt{\mu}_{\nu}$:
\begin{corollary}\label{co:closed-loop.closure.M}
Let $A - B V_{22} V_{21}^{-1}$ and $B$ be full (column) rank. Then, for all $\nu \geq 0$, $\lim_{\mu \rightarrow \wt{\mu}_{\nu}} \rho(A^c_{\mu,\nu}) = 1$.
%\begin{equation*}
%\lim_{\mu \rightarrow \wt{\mu}_{\nu}} \rho(A^c_{\mu,\nu}) \rightarrow 1.
%\end{equation*}
\end{corollary}
The proof of Cor.~\ref{co:closed-loop.closure.M} is straightforward, since by contradiction, if $\lim_{\mu \rightarrow \wt{\mu}_{\nu}} \rho(A^c_{\mu,\nu}) < 1$, then for all $K$, $\Psi_{\mu,\nu}^K(z) \succ 0$ on the unit circle $|z| = 1$, which is not possible from the definition of $\wt{\mu}_\nu$ (see Eq.~\ref{eq:mutilde.definition}).\\

 In essence, Lem.~\ref{le:existence.closure.M} relies on the behavior of $D_{\mu,\nu} = R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B}$ when $\mu \rightarrow \wt{\mu}_{\nu}$. Now that the existence of $P_{\mu,\nu}$ is asserted on $\wb{\mathcal{M}}$, Lem.~\ref{le:positivity.margin} exhibits the relationship between $D_{\mu,\nu} \succ 0$ and  $A - B V_{22} V_{21}^{-1}$ and $B$ be full (column) rank.

\begin{lemma}\label{le:positivity.margin}
Let $A - B V_{22} V_{21}^{-1}$ and $B$ be full (column) rank. Then, for all $(\mu,\nu) \in \wb{\mathcal{M}}$ such that $\|K_{\mu,\nu}\|_2 \leq c < \infty$, $D_\mu \succcurlyeq \alpha I$, where 
\begin{equation*}
\begin{aligned}
&\alpha =  \min\left(  \frac{c_2}{(c_1 c_2)^{n+d}} \min \left( c_3, \frac{\wb{\epsilon} \alpha_{\min}}{c_2} \right),\frac{\lambda_{\min}(H)}{4 \max\big(2,1 + 2 \|B\|_2^2)}\right), \\
&c_1 = 1 + \Big( (\|A\|_2 + c )\|\tilde{B}\|_2 \Big)^2; \quad c_2 =\max\big( \lambda_{\max}(R), \tilde{\mu}\big) + (D + n \tilde{\mu}) \|\tilde{B}\|_2^2; \quad c_3 = (\mu_+ \alpha_{\min}(B))/2,\\
&\alpha_{\min} = \mu_+ \big( 1 + (1 + \|B V_{22}\|)^2 \big)^{-1/2} \big( 1 + (1 + \|V_{21}^{-1} V_{22}\|)^2 \big)^{-1/2} \min\Big( \sigma_{\min}\big( A - B V_{22} V_{21}^{-1} \big),\lambda_{\min}(V_{22}^{-1}) \Big),\\
&\alpha_{\min}(B) = \frac{\sigma_{\min}(B)^2}{2 (2 + \sigma_{\min}(B)^2)}; \quad 
\wb{\epsilon} = \min \left( \alpha_{\min}(B),  \frac{\mu_+ \alpha_{\min}(B)}{2 (D + n \tilde{\mu}))}\right).\\
&\mu_+ \text{ is the solution of } \lambda_{\min}(H_{\mu_+}) = \lambda_{\min} \left( H - \mu_+ V^{-1} \right) = 1/2 \lambda_{\min}(H)
\end{aligned}
\end{equation*}
\end{lemma}

The proofs of Lem.~\ref{le:existence.closure.M} and~\ref{le:positivity.margin} relies intensively on the Popov function properties and are postpone to App.~\ref{sec:app.popov.positivity}.


\subsection{Characterization of $\D(\mu)$}\label{ssec:app.proof.extended.riccati1}

We now characterize further the dual function $\mathcal{D}$ w.r.t. the Lagrangian parameters $(\mu,\nu) \in \mathcal{M}$. We first recall that by construction, the dual function $\mathcal{D}$ is concave (i.e., it is the minimum of affine functions) and that by Property.~\ref{prop:domain.mutilde.nu}, $\mathcal{M}$ is a convex set. Therefore, Alexandrov's Theorem guarantees that $\mathcal{D}$ is twice differentiable \textit{almost everywhere} on $\mathcal{M}$. Moreover, the following property ensures that the only points of discontinuity lies possibly on the frontier of $\mathcal{M}$ i.e., on $\{ (\wt{\mu}_\nu, \nu), \hspace{1mm} \nu \geq 0\}$ and hence that $\mathcal{D}$ is twice differentiable  \textit{everywhere} on the interior of $\mathcal{M}$.

\begin{property}\label{prop:domain.characterization.1}
For all $(\mu,\nu)$ in the interior of $\mathcal{M}$, $\mathcal{D}(\mu) > -\infty$.
\end{property}
\begin{proof}
For all $\nu < +\infty$, for all $\mu < \min(\wt{\mu}_{\nu}, +\infty)$, $R_\mu \prec + \infty$. Thus, taking the trace of the first condition in Eq.~\ref{eq:admissible.riccati.solution} leads to:
\begin{equation*}
\Tr( P_\mu \wt{B} \wt{B}^\transp) \geq - \Tr(R_\mu) \quad \Rightarrow \quad \Tr\big( P_\mu(I + B B^\transp)\big) > - \Tr(R_\mu) \quad  \Rightarrow \quad \Tr(P_\mu) > - \infty.
\end{equation*}
\end{proof}

The following property provides an explicit characterization of the derivative of a Riccati solution w.r.t. the cost matrix as unique solution of Discrete Lyapunov equation.
\begin{property}
\label{prop:derivative.riccati.cost.matrix}
For any $(\mu,\nu) \in \mathcal{M}$, let $d_\mu P_{\mu,\nu}$ and $d_\nu P_{\mu,\nu}$ the (matrix) partial derivative w.r.t. $\mu$ and $\nu$ respectively. Then,
\begin{equation}
\label{eq:derivative.riccati.cost.matrix}
\begin{aligned}
d_\mu P_{\mu,\nu} &= \big( A^c_{\mu,\nu}\big)^\transp d_\mu P_{\mu,\nu} A^c_{\mu,\nu} + \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}^\transp \begin{pmatrix} - V^{-1} & 0 \\ 0 & I \end{pmatrix}\begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix} \\
\vspace{5cm}
d_\nu P_{\mu,\nu} &= \big( A^c_{\mu,\nu}\big)^\transp d_\nu P_{\mu,\nu} A^c_{\mu,\nu} + \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}^\transp \begin{pmatrix} K_0^\transp K_0 & -K_0^\transp & 0 \\ -K_0 & I & 0 \\ 0 & 0 & 0 \end{pmatrix} \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}.
\end{aligned}
\end{equation}
\end{property}

%\begin{proof}[Proof of Property.~\ref{prop:derivative.riccati.cost.matrix}]
The proof follows from a direct (matrix) differentiation of Eq.~\ref{eq:admissible.riccati.solution} w.r.t. $\mu$ and $\nu$. 
%Since it works exactly the same for $\mu$ and $\nu$, we only report here the derivation w.r.t. $\mu$. From 
\begin{equation*}
P_{\mu,\nu} = Q_{\mu,\nu} + A^\transp P_{\mu,\nu} A  - [ A^\transp P_{\mu,\nu} \tilde{B} + N_{\mu,\nu}^\transp ] [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1} [ \tilde{B}^\transp P_{\mu,\nu} A + N_{\mu,\nu} ].
\end{equation*}
%we obtain:
%\begin{equation*}
%\begin{aligned}
%d_\mu P_{\mu,\nu} &= d_\mu Q_{\mu,\nu} + A^\transp d_\mu P_{\mu,\nu} A   - [ A^\transp d_\mu P_{\mu,\nu} \tilde{B} + d_\mu N_{\mu,\nu}^\transp ] [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1} [ \tilde{B}^\transp P_{\mu,\nu} A + N_{\mu,\nu} ]  \\
%&- [ A^\transp P_{\mu,\nu} \tilde{B} + N_{\mu,\nu}^\transp ] [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1} [ \tilde{B}^\transp d_\mu P_{\mu,\nu} A + d_\mu N_{\mu,\nu} ]  \\
%&+ [ A^\transp d_\mu P_{\mu,\nu} \tilde{B} + d_\mu N_{\mu,\nu}^\transp ] [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1}  [ d_\mu R_{\mu,\nu} + \tilde{B}^\transp d_\mu P_{\mu,\nu} \tilde{B} ] [ R_{\mu,\nu} + \tilde{B}^\transp P_{\mu,\nu} \tilde{B} ]^{-1}  [ \tilde{B}^\transp P_{\mu,\nu} A + N_{\mu,\nu} ]  \\
%&= d_\mu Q_{\mu,\nu} + A^\transp d_\mu P_{\mu,\nu} A   +  [ A^\transp d_\mu P_{\mu,\nu} \tilde{B} + d_\mu N_{\mu,\nu}^\transp ] K_{\mu,\nu} + K_{\mu,\nu}^\transp [ \tilde{B}^\transp d_\mu P_{\mu,\nu} A + d_\mu N_{\mu,\nu} ]  \\
%&+ K_{\mu,\nu}^\transp [ d_\mu R_{\mu,\nu} + \tilde{B}^\transp d_\mu P_{\mu,\nu} \tilde{B} ] K_{\mu,\nu} \\
%&= d_\mu Q_{\mu,\nu} + A^\transp d_\mu P_{\mu,\nu} A^c_{\mu,\nu}   + K_{\mu,\nu}^\transp \tilde{B}^\transp d_\mu P_{\mu,\nu} A^c_{\mu,\nu}  + K_{\mu,\nu}^\transp d_\mu N_{\mu,\nu}  +  d_\mu N_{\mu,\nu}^\transp  K_{\mu,\nu}  + K_{\mu,\nu}^\transp d_\mu R_{\mu,\nu} K_{\mu,\nu} \\
%&= \big( A^c_{\mu,\nu} \big)^\transp d_\mu P_{\mu,\nu} A^c_{\mu,\nu}  + K_{\mu,\nu}^\transp d_\mu N_{\mu,\nu}  +  d_\mu N_{\mu,\nu}^\transp  K_{\mu,\nu}  + K_{\mu,\nu}^\transp d_\mu R_{\mu,\nu} K_{\mu,\nu} \\
%&= \big( A^c_{\mu,\nu}\big)^\transp d_\mu P_{\mu,\nu} A^c_{\mu,\nu} + \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}^\transp d_\mu H_{\mu,\nu} \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}
%\end{aligned}
%\end{equation*}
%Finally, the linearity of $H_{\mu,\nu}$ leads to $d_\mu H_{\mu,\nu}  = \begin{pmatrix} - V^{-1} & 0 \\ 0 & I \end{pmatrix}$ which concludes the proof.
%\end{proof}


\begin{proof}[proof of Prop.~\ref{p:function.D}]
Thanks to Property.~\ref{prop:derivative.riccati.cost.matrix}, one has 
\begin{equation}
\label{eq:derivative.dual.mu.nu.1}
\mathcal{D}^\prime_\mu( \mu,\nu) = \Tr( d_\mu P_{\mu,\nu} ); \quad \mathcal{D}^\prime_\nu( \mu,\nu) = \Tr( d_\nu P_{\mu,\nu} ) - \big( \epsilon_0^{u} \big)^2
\end{equation}
where $d_\mu P_{\mu,\nu}$ and $d_\nu P_{\mu,\nu}$ are defined in Eq.~\ref{eq:derivative.riccati.cost.matrix}. Further, let $\Sigma_{\mu,\nu}$ be the steady-state variance of the state process $x_{s+1} =  A^c_{\mu,\nu} x_s + \epsilon_{s+1}$, one has:
\begin{equation*}
\Sigma_{\mu,\nu} =  \big( A^c_{\mu,\nu}\big)^\transp  \Sigma_{\mu,\nu} A^c_{\mu,\nu} + I.
\end{equation*}
Standard Riccati manipulations then leads to:
\begin{equation*}
\begin{aligned}
\Tr( d_\mu P_{\mu,\nu} ) &=  \Tr \left(  \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}^\transp \begin{pmatrix} - V^{-1} & 0 \\ 0 & I \end{pmatrix}\begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix} \Sigma_{\mu,\nu}\right)\\
\Tr( d_\nu P_{\mu,\nu} ) &=  \Tr \left( \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}^\transp \begin{pmatrix} K_0^\transp K_0 & -K_0^\transp & 0 \\ -K_0 & I & 0 \\ 0 & 0 & 0 \end{pmatrix} \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix} \Sigma_{\mu,\nu}\right)
\end{aligned}
\end{equation*}
Finally, using $\Sigma_{\mu,\nu} = \lim_{S \rightarrow \infty} \frac{1}{S} \mathbb{E} \left( \sum_{s=1}^S x_s x_s^\transp \right)$, that $K_{\mu,\nu} x_s = \begin{pmatrix} u_s \\ w_s \end{pmatrix}$ and that $z_s = \begin{pmatrix} x_s \\ u_s \end{pmatrix}$ one obtains:
\begin{equation}
\label{eq:from.gradient.to.constraints}
\begin{aligned}
\mathcal{D}^\prime_\mu( \mu,\nu) &=    \lim_{S \rightarrow \infty} \frac{1}{S}  \mathbb{E} \Big( \sum_{s=0}^S\|w_s \|^2 -  \| z_s \|^2_{V^{-1}} \Big) = g_{\tpi_{\mu,\nu}} \\
 \mathcal{D}^\prime_\nu( \mu,\nu) &=  \lim_{S \rightarrow \infty} \frac{1}{S}  \mathbb{E} \Big( \sum_{s=0}^S\| u_s - K_0 x_s\|^2 \Big) - (\epsilon_0^u)^2 = h_{\tpi_{\mu,\nu}}  \\
\end{aligned}
\end{equation}
which proves the first two statements of Prop.~\ref{p:function.D}. Additionally, we obtain the following relationship between $\mathcal{D}$ and its derivative:
\begin{equation}
\label{eq:dual.constraints.derivatives}
 \mathcal{D}(\mu,\nu) = \mathcal{J}_{\tpi_{\mu,\nu}}  + \mu g_{\tpi_{\mu,\nu}} + \nu h_{\tpi_{\mu,\nu}} =  \mathcal{J}_{\tpi_{\mu,\nu}} + \mu \mathcal{D}^\prime_\mu( \mu,\nu) + \nu  \mathcal{D}^\prime_\nu( \mu,\nu)
\end{equation}
where $\mathcal{J}_{\tpi_{\mu,\nu}}$ is the cost of the extended linear system induced by the controller $K_{\mu,\nu}$. Formally, 
\begin{equation}
\label{eq:true.extended.cost.riccati}
\mathcal{J}_{\tpi_{\mu,\nu}} = \Tr\big(P(K_{\mu,\nu}) \big) \quad \text{ where } \quad P(K_{\mu,\nu}) =  \big(A^c_{\mu,\nu}\big)^{\transp} P(K_{\mu,\nu}) A^c_{\mu,\nu} + \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}^\transp \begin{pmatrix} Q & 0 &0 \\ 0 & R &0 \\ 0 & 0 &0 \end{pmatrix} \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}.
\end{equation}

To obtain the second derivative w.r.t. $\mu$, we differentiate further Eq.~\ref{eq:derivative.dual.mu.nu.1} and get:
\begin{equation}
\label{eq:second.derivative.riccati.mu}
\mathcal{D}^{\prime \prime}_{\mu}(\mu,\nu) = \Tr\big( d^2_\mu  P_{\mu,\nu}\big); \quad \quad
d^2_\mu P_{\mu,\nu} = \big( A^c_{\mu,\nu}\big)^\transp d^2_\mu P_{\mu,\nu} A^c_{\mu,\nu}  - \frac{2}{\mu^2} Y_{\mu,\nu}^\transp [R_{\mu,\nu} + \wt{B}^\transp P_{\mu,\nu} \wt{B} ]^{-1} Y_{\mu,\nu},
\end{equation}
where 
\begin{equation*}
\begin{aligned}
Y_{\mu,\nu} &= \big( R_{0,\nu} + \wt{B}^\transp P_{0,\nu}(K_{\mu,\nu}) \wt{B} \big) K_{\mu,\nu} + \wt{B}^\transp P_{0,\nu}(K_{\mu,\nu}) A + N_{0,\nu},\\
P_{0,\nu}(K_{\mu,\nu}) &=  \big( A^c_{\mu,\nu}\big)^\transp P_{0,\nu}(K_{\mu,\nu}) A^c_{\mu,\nu} + \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix}^\transp H_{0,\nu} \begin{pmatrix} I \\ K_{\mu,\nu} \end{pmatrix},\\
\end{aligned}
\end{equation*}
Clearly, $H_{0,\nu}$ is p.s.d. since it consists in the strictly p.s.d. part of $H_{\mu,\nu}$. As a result, so is $P_{0,\nu}(K_{\mu,\nu})$. Futher, since for all $(\mu,\nu) \in \mathcal{M}$, $R_{\mu,\nu} + \wt{B}^\transp P_{\mu,\nu} \wt{B}$ is p.s.d. and so is $-d^2_\mu P_{\mu,\nu}$. Thus, $\mathcal{D}^{\prime \prime}_{\mu}(\mu,\nu) \leq 0$, which is expected as $\mathcal{D}$ is concave.\\


We now show that for any $\nu \geq 0$, $\mu \rightarrow \mathcal{D}(\mu,\nu)$ admits a unique global supremum (potentially at infinity). The idea of the proof is the following: either $\mathcal{D}^\prime_\mu(0,\nu) < 0$, thus the maximum is unique by concavity and is attained at $\mu = 0$, either the maximum is not attained at $0$ and $\mu \rightarrow \mathcal{D}(\mu,\nu)$ is strictly concave, thus it admits a unique global supremum (potentially at infinity).\\ 
For any $\nu \geq 0$, suppose that it exists $\mu > 0$ such that $\mathcal{D}^{\prime \prime}_\mu(\mu,\nu) = 0$. Then, $d^2_\mu P_{\mu,\nu} = 0$ which is equivalent to $Y_{\mu,\nu} = 0$. Further, $Y_{\mu,\nu} = 0$ if and only if $K_{\mu,\nu} = K_{0,\nu}$. let $K_{0,\nu} = \begin{pmatrix} K^{u}_{0,\nu}\\ K_{0,\nu}^{w} \end{pmatrix}$ be block decomposition associated with control $u$ and perturbation $w$, then, it is easy to show that $K_{0,\nu}^{w} = -(A + B K^{u}_{0,\nu})$ since the optimal unconstrained choice of the perturbation is to cancel completely the closed-loop matrix induced by the control. Futher, algebraic manipulation show that:
\begin{equation*}
K_{\mu,\nu}^{w} = - (P_{\mu,\nu} + \mu I)^{-1} P_{\mu,\nu} \theta^\transp \begin{pmatrix} I \\ K_{\mu,\nu}^{u} \end{pmatrix} \quad \quad \Leftrightarrow \quad\quad  K_{0,\nu}^{w} = - (P_{\mu,\nu} + \mu I)^{-1} P_{\mu,\nu} \theta^\transp \begin{pmatrix} I \\ K_{0,\nu}^{u} \end{pmatrix},
\end{equation*}
which translates into 
\begin{equation*}
\begin{aligned}
A + B K^{u}_{0,\nu} = (P_{\mu,\nu} + \mu I)^{-1} P_{\mu,\nu} ( A + B K^{u}_{0,\nu}) \quad &\Leftrightarrow \quad (P_{\mu,\nu} + \mu I) ( A + B K^{u}_{0,\nu}) = P_{\mu,\nu} (A + B K^{u}_{0,\nu}) \\
&\Leftrightarrow \quad\quad \mu ( A + B K^{u}_{0,\nu}) = 0  \quad\quad \Leftrightarrow  A + B K^{u}_{0,\nu} = 0.
\end{aligned}
\end{equation*}
As a result, 
\begin{enumerate}
\item either $A + B K^{u}_{0,\nu} = 0$ and $K_{0,\nu}^{w} = 0$ thus $\Tr(d_\mu P_{0,\nu}) \leq - \Tr(V_{11}^{-1}) < 0$ and the maximum is attained at $0$,
\item either $A + B K^{u}_{0,\nu} \neq 0$ and we obtain that $\mu \rightarrow \mathcal{D}(\mu,\nu)$ is strictly concave (by contradiction).
\end{enumerate}
%
%Suppose that it exists $(\bar{\mu},\bar{\nu}) \in \mathcal{M}$ such that $\mathcal{D}^{\prime \prime}_\mu(\bar{\mu},\bar{\nu}) = 0$. Then, $d^2_\mu P_{\bar{\mu},\bar{\nu}} = 0$ which is equivalent to $Y_{\bar{\mu},\bar{\nu}} = 0$. Further, $Y_{\bar{\mu},\bar{\nu}} = 0$ if and only if $K_{\bar{\mu},\bar{\nu}} = K_{0,\bar{\nu}}$. As a result, we just have to show that for all $\nu \in \mathbb{R}_+$, $K_{\mu,\nu} \neq K_{0,\nu}$ to guarantee strict concavity.\\
%First, notice that for all $\nu$, $K_{0,\nu} = \begin{pmatrix} K_0 \\ -(A + B K_0 ) \end{pmatrix}$. Further, for all $(\mu,\nu) \in \mathcal{M}$, let $K_{\mu,\nu} = \begin{pmatrix} K^{u}_{\mu,\nu}\\ K_{\mu,\nu}^{w} \end{pmatrix}$ be block decomposition associated with control $u$ and perturbation $w$, then, algebraic manipulation show that:
%\begin{equation*}
%K_{\mu,\nu}^{w} = - (P_{\mu,\nu} + \mu I)^{-1} P_{\mu,\nu} \theta^\transp \begin{pmatrix} I \\ K_{\mu,\nu}^{u} \end{pmatrix}.
%\end{equation*}
%Hence, $K_{\mu,\nu} = K_{0,\nu}$ if and only if $K_{\mu,\nu}^{u} = K_0$ and $K^{w}_{\mu,\nu} = K_{0,\nu}^{w}$ thus necessarily,
%\begin{equation*}
%\begin{aligned}
%A + B K_0 = (P_{\mu,\nu} + \mu I)^{-1} P_{\mu,\nu} ( A + B K_0) \quad &\Leftrightarrow \quad (P_{\mu,\nu} + \mu I) ( A + B K_0) = P_{\mu,\nu} (A + B K_0) \\
%&\Leftrightarrow \quad \mu ( A + B K_0) = 0
%\end{aligned}
%\end{equation*}
%Therefore, either $A + B K_0 = 0$ and $(0,0) \in \arg\max_{(\mu,\nu) \in \mathcal{M}} \mathcal{D}(\mu,\nu)$ (notice that the set of $(A,B)$ satisfying this equality is of zero Lesbegue measure), either $A + B K_0 \neq 0$ and by contradiction, $\mathcal{D}(\mu,\nu)$ is strictly concave w.r.t. $\mu$. This proves the third statement of Prop.~\ref{p:function.D} and concludes the proof.
\end{proof}

We are now ready to prove the core statement of Lem.~\ref{lem:dual.function}.2.

\subsection{Proof of Lemma~\ref{lem:dual.function}.2}


While Lemma.~\ref{lem:dual.function}.1 certifies the existence of a domain $\mathcal{M}$ where $\D(\mu,\nu)$ can be efficiently computed by solving a Riccati equation, it does not provide any guarantee on whether the supremum of $\D(\mu,\nu)$ is actually attained \textit{within} $\mathcal{M}$. \\

We first recall that by construction, the dual function $\mathcal{D}$ is concave (i.e., it is the minimum of affine functions) and that by Property.~\ref{prop:domain.mutilde.nu}, $\mathcal{M}$ is a convex set. Intuitively, we prove the statement of Lemma~\ref{lem:dual.function}.2) by showing that for any $\nu \geq 0$, there exists at least one point of non-positive derivative w.r.t. $\mu$ within $[0,\wt\mu_\nu)$. In fact, by concavity, this would imply that the maximum in attained in $[0,\wt\mu_\nu)$. The following proposition then guarantees the existence of at least one point of non-positive derivative within $[0,\wt\mu_\nu)$.

\begin{proposition}\label{p:infinite_gradient}
Let $A - B V_{22} V_{21}^{-1}$ and $B$ be full (column) rank. For any $\nu \geq 0$, let $\wt{\mu}_\nu$ be defined by Eq.~\eqref{eq:mutilde.definition}, one has that 
\begin{equation*}
\lim_{\mu \rightarrow \wt{\mu}_\nu} \mathcal{D}^\prime_\mu(\mu,\nu) = - \infty.
\end{equation*}
\end{proposition}

\begin{proof}
Thanks to Prop.~\ref{p:function.D}, we have that $\mathcal{D}$ is twice differentiable on $[0,\wt{\mu}_\nu)$ for any $\nu \geq 0$. Further, Cor.~\ref{co:closed-loop.closure.M} ensures that $\lim_{\mu \rightarrow \wt{\mu}_\nu} \rho\big(A^c_{\mu,\nu}\big) = 1$. Thus, let $P(K_{\mu,\nu})$ be defined as in Eq.~\ref{eq:true.extended.cost.riccati}, standard Lyapunov result implies that 
\begin{equation*}
\lim_{\mu \rightarrow \wt{\mu}_\nu} \Tr\big(P(K_{\mu,\nu})\big) = + \infty.
\end{equation*}
However, recalling Eq.~\ref{eq:dual.constraints.derivatives}, 
\begin{equation*}
 \mathcal{D}(\mu,\nu) = \Tr\big(P(K_{\mu,\nu})\big) + \mu \mathcal{D}^\prime_\mu( \mu,\nu) + \nu  \mathcal{D}^\prime_\nu( \mu,\nu)
\end{equation*}
and $\mathcal{D}(\mu,\nu) \leq D < + \infty$ by weak duality. Finally, it is clear from Eq.~\ref{eq:from.gradient.to.constraints} that $\mathcal{D}^\prime_\nu( \mu,\nu) \geq - \big(\epsilon_0^{u}\big)^2 > -\infty$, thus necessarily,
\begin{equation*}
\lim_{\mu \rightarrow \wt{\mu}_\nu} \mathcal{D}^\prime_\mu( \mu,\nu)   = - \infty.
\end{equation*}
\end{proof}
As a result, by continuity, for any $\nu \geq 0$ it exists $\mu^*_\nu \in [0,\wt{\mu}_\nu)$ such that $\mathcal{D}^\prime_\mu(\mu^*_\nu,\nu) \leq 0$. This implies that the maximum is attained in $[0,\wt{\mu}_\nu)$ and conclude the proof of Lemma~\ref{lem:dual.function}.2.

\subsection{Proof of Theorem~\ref{thm:dual.gap}}

The strong duality result directly follows from Lem.~\ref{lem:dual.function} which ensures that for any $\nu \geq 0$, the function $\mu \rightarrow \mathcal{D}(\mu,\nu)$ attains it maximum on the interior of $\mathcal{M}$. Let $(\mu^*,\nu^*)$ be a point at which the maximum is attained, the following situation can occur:
\begin{enumerate}
\item either, $\mathcal{D}^\prime_\mu(\mu^*,\nu^*) = 0$ and $\mathcal{D}^\prime_\nu(\mu^*,\nu^*) = 0$,
\item either, $\mu^* = 0$, $\nu^* > 0$ and $\mathcal{D}^\prime_\mu(\mu^*,\nu^*) \leq 0$, $\mathcal{D}^\prime_\nu(\mu^*,\nu^*) = 0$,
\item either, $\nu^* = 0$, $\mu^* > 0$ and $\mathcal{D}^\prime_\mu(\mu^*,\nu^*) = 0$, $\mathcal{D}^\prime_\nu(\mu^*,\nu^*) \leq 0$,
\item either, $\mu^* = 0$ and $\nu^* = 0$.
\end{enumerate}
Immediately, this translates into the primal feasability and complementary slackness conditions by Prop.~\ref{p:function.D}:
\begin{equation*}
g_{\tpi_{\mu^*,\nu^*}} \leq 0; \quad h_{\tpi_{\mu^*,\nu^*}}  \leq 0 \quad \text{ and } \quad \mu^*  g_{\tpi_{\mu^*,\nu^*}} = \nu^* h_{\tpi_{\mu^*,\nu^*}}  = 0.
\end{equation*}

As a result, from Eq.~\ref{eq:dual.constraints.derivatives}, 
\begin{equation*}
\mathcal{D}(\mu^*,\nu^*) = \mathcal{J}_{\tpi_{\mu^*,\nu^*}}  + \mu^* g_{\tpi_{\mu^*,\nu^*}} + \nu^* h_{\tpi_{\mu^*,\nu^*}} = \mathcal{J}_{\tpi_{\mu^*,\nu^*}} \geq \mathcal{J}_*.
\end{equation*}
On the other hand, weak duality guarantees that $\mathcal{D}(\mu^*,\nu^*) \leq \mathcal{J}_*$ which leads to $\mathcal{D}(\mu^*,\nu^*) = \mathcal{J}_*$ thus proving that strong duality holds.

\subsection{Range for $\nu_{\max}$ and $\mu_{\max}$}\label{ssec:app.proof.range}
We conclude this section with the proof of Prop.~\ref{p:bounding.mu.nu} which allows us to restrict the search for $(\mu^*,\nu^*)$ over $\mathcal{M} \cap \big\{ [0, \mu_{\max}] \times [0,\nu_{\max}] \big\}$.
\begin{proof}
From Thm.~\ref{thm:dual.gap}, we have that $\mathcal{D}(\mu_*,\nu_*) = \max_{(\mu,\nu) \in \mathbb{R}_+^2} \mathcal{D}(\mu,\nu) = \mathcal{J}_{*}(\wh\theta, \beta, V, \Theta_0) > 0$. On the other hand, for any $(\mu,\nu) \in \mathbb{R}_+^2$, $\mathcal{D}(\mu,\nu) =  \min_{\tpi} \mathcal L_{\tpi}(\mu, \nu)$. As a result, considering the policy $\tpi_0(x) = \big( K_0 x, 0 \big)$, one gets:
\begin{equation*}
\mathcal{D}(\mu,\nu) \leq \mathcal{J}_{\tpi_0}(\wh\theta) + \mu g_{\tpi_0}(\wh\theta,\beta, V) + \nu h_{\tpi_0}(\wh\theta, \Theta_0).
\end{equation*}
Further, $g_{\tpi_0}(\wh\theta,\beta, V) < 0$ as the policy $\tpi_0$ does not induce any perturbations $w$, while $h_{\tpi_0}(\wh\theta, \Theta_0) = \nu (\epsilon_0^{u})^2$. We now conclude the proof by contradiction:
\begin{itemize}
\item suppose that $\nu_{*} \geq \nu_{\max}$. Then, $0 < \mathcal{D}(\mu_*,\nu_*) \leq  \mathcal{J}_{\tpi_0}(\wh\theta) -  \nu_* (\epsilon_0^{u})^2 \leq \mathcal{J}_{\tpi_0}(\wh\theta) -  \nu_{\max} (\epsilon_0^{u})^2 \leq 0$.
\item suppose that $\mu_* \geq \mu_{\max}$. Then, $0 < \mathcal{D}(\mu_*,\nu_*) \leq  \mathcal{J}_{\tpi_0}(\wh\theta)+ \mu_* g_{\tpi_0}(\wh\theta,\beta, V)  \leq \mathcal{J}_{\tpi_0}(\wh\theta) -  \mu_{\max} g_{\tpi_0} \leq 0$.
\end{itemize}

\end{proof}




\section{Proof of Lem.~\ref{le:existence.closure.M} and~\ref{le:positivity.margin}}\label{sec:app.popov.positivity} 

The proofs of Lem.~\ref{le:existence.closure.M} and~\ref{le:positivity.margin} address the limit behavior of the Riccati solution of Eq.~\ref{eq:admissible.riccati.solution} and $D_{\mu,\nu}$ respectively. We first reparametrize the LQR problem~\ref{eq:extended.lqr.definition.mu.nu} to isolate the difficulty (contained in $\mu$) and then provide the proofs for $\nu = 0$ without loss of generality. As in App.~\ref{sec:app.proof.duality}, we consider without loss of generality that $\beta = 1$ for sake of readability. Finally, we assume throughout all this section that $A - B V_{22} V_{21}^{-1}$ is full rank and $B$ is full column rank.

\subsection{Reparametrization} When $\nu$ is fixed, we can discard the constant term $- \nu(\epsilon_0^u)^2$ in the LQR problem~\ref{eq:extended.lqr.definition.mu.nu} without affecting the minimization and maximization properties. Furthermore, the matrix $H_\nu$ is p.s.d.\ and thus it contributes towards ``more standard'' LQR systems with p.s.d.\ cost matrices $H_{\mu,\nu}$. Since the main technical difficulty with the analysis is to characterize the behaviour of $\D(\mu,\nu)$ for values of $\mu$ where ``standard'' Riccati theory does not hold, without loss of generality with only focus on the case $\nu=0$. This is supported by the fact that the problem is invariant under reparametrization of $\wt{u}$. Using the reparametrization $u_s = \nu (R + \nu I)^{-1} K_0 x_s + \wb{u}_s$ and overloading notation by denoting $\wt{u}_s = [\wb{u}_s^\transp, w_s^\transp]^\transp$, one obtains an equiavelent reformulation of the LQR problem~\ref{eq:extended.lqr.definition.mu.nu} as:
\begin{equation*}
\begin{aligned}
\mathcal L_{\tpi}(\mu, \nu) &=\lim_{S \rightarrow \infty} \frac{1}{S} \mathbb{E} \bigg[ \sum_{s=0}^{S-1} \begin{pmatrix} x_s^\transp & \tilde{u}_s^\transp \end{pmatrix} \wb{H}_{\mu} \begin{pmatrix} x_s \\ \tilde{u}_s \end{pmatrix} \bigg]\\
\text{subject to } &x_{s+1} = \wb{A} x_s + \wt{B} \wt{u}_s+ \epsilon_{s+1}
\end{aligned}
\end{equation*}
where 
\begin{equation*}
\begin{aligned}
&\wb{H}_{\mu} = \wb{H} + \wb{H}_{\mu}; \quad \wb{A} = A + \nu B(R + \nu I)^{-1} K_0; \quad \wb{H} =\begin{pmatrix} \wb{Q} & 0 & 0\\ 0 & \wb{R} & 0 \\ 0 & 0 & 0 \end{pmatrix}; \quad \wb{H}_\mu = \mu \begin{pmatrix} - \wb{V}^{-1} & 0 \\ 0 & I \end{pmatrix} \\
&\wb{Q} = Q - \nu^2 K_0^\transp (R + \nu I)^{-1}K_0; \quad \wb{R} = R + \nu I; \quad \wb{V}^{-1} =  \begin{pmatrix} I & \nu K_0^\transp (R+\nu I)^{-1} \\ 0 & I \end{pmatrix} V^{-1}  \begin{pmatrix} I & 0\\ \nu (R+\nu I)^{-1}K_0  & I \end{pmatrix}.
\end{aligned}
\end{equation*}
The linear parametrization does not affect positive definiteness properties, thus $\wb{V}^{-1}$ is p.s.d. Further, $\wb{Q}$ is also p.s.d since $\wb{H}$ is p.s.d, which can be easily checked from:
$$\bar{H} = \begin{pmatrix} I & \nu K_0^\transp (R+\nu I)^{-1} \\ 0 & I \end{pmatrix} (H^\dagger + H_\nu ) \begin{pmatrix} I & 0\\ \nu (R+\nu I)^{-1}K_0  & I \end{pmatrix}.$$
Finally, let $$ V^{-1} := \begin{pmatrix} V_{11}^{-1} & V_{12}^{-1} \\ V_{21}^{-1} & V_{22}^{-1} \end{pmatrix}; \quad \wb{V}^{-1} := \begin{pmatrix} \wb{V}_{11}^{-1} & \wb{V}_{12}^{-1} \\ \wb{V}_{21}^{-1} & \wb{V}_{22}^{-1} \end{pmatrix}$$ be the block decomposition of $ V^{-1}$ and $\wb{V}^{-1}$ with blocks corresponding to states $x$ and controls $u$. The condition $A - B V_{22} V_{21}^{-1}$ is full rank ensures that, for all $\nu > 0$,
\begin{equation*}
\ker(\wb{A}) \cap \ker(\wb{V}_{21}^{-1}) = \{ 0 \}.
\end{equation*}

\begin{property}
\label{prop:reparametrization.full.rank}
For any $\nu \geq 0$, let $\wb{A}$ and $ \wb{V}^{-1}$ be the reparametrized matrices. Then,
\begin{equation*}
\sigma_{\min}\begin{pmatrix} \wb{A} \\ \wb{V}_{21}^{-1} \end{pmatrix} \geq  \big( 1 + (1 + \|B V_{22}\|)^2 \big)^{-1/2} \big( 1 + (1 + \|V_{21}^{-1} V_{22}\|)^2 \big)^{-1/2} \min\Big( \sigma_{\min}\big( A - B V_{22} V_{21}^{-1} \big),\lambda_{\min}(V_{22}^{-1}) \Big).
\end{equation*}
\end{property}
\begin{proof}
The proof relies on Schur complement decomposition of block matrices and standard singular/eigenvalue properties. First, notice that 
\begin{equation*}
\begin{pmatrix} \wb{A} \\ \wb{V}_{21}^{-1} \end{pmatrix} = \begin{pmatrix} A & B \\ V_{21}^{-1} & V_{22}^{-1} \end{pmatrix} \begin{pmatrix} I \\  -( R + \nu I)^{-1} K_0 \end{pmatrix}
\end{equation*}
which immediately implies that $\sigma_{\min} \begin{pmatrix} \wb{A} \\ \wb{V}_{21}^{-1} \end{pmatrix}  \geq \sigma_{\min} \begin{pmatrix} A & B \\ V_{21}^{-1} & V_{22}^{-1} \end{pmatrix}$ for which we provide a lower bound.\\
From $V_{22}^{-1} \succ 0$ we have,
\begin{equation*}
 \begin{pmatrix} A & B \\ V_{21}^{-1} & V_{22}^{-1} \end{pmatrix} =  \begin{pmatrix} I & B V_{22} \\ 0 & I \end{pmatrix}   \begin{pmatrix} A - B V_{22} V_{21}^{-1} & 0 \\ 0 & V_{22}^{-1} \end{pmatrix}   \begin{pmatrix} I & 0 \\ V_{22} V_{21}^{-1} & I \end{pmatrix}.
\end{equation*}
Moreover, 
\begin{equation*}
\sigma_{\min} \begin{pmatrix} I & 0 \\ V_{22} V_{21}^{-1} & I \end{pmatrix} \geq  \big( 1 + (1 + \|V_{21}^{-1} V_{22}\|)^2 \big)^{-1} \quad \text{ and } \quad 
\sigma_{\min} \begin{pmatrix} I & B V_{22} \\ 0 & I \end{pmatrix}  \geq  \big( 1 + (1 + \|B V_{22}\|)^2 \big)^{-1}.
\end{equation*}
Finally, the proof is concluded using that
\begin{equation*}
\sigma_{\min}  \begin{pmatrix} A & B \\ V_{21}^{-1} & V_{22}^{-1} \end{pmatrix} \geq \sigma_{\min} \begin{pmatrix} I & B V_{22} \\ 0 & I \end{pmatrix} \sigma_{\min} \begin{pmatrix} I & 0 \\ V_{22} V_{21}^{-1} & I \end{pmatrix} \sigma_{\min} \begin{pmatrix} A - B V_{22} V_{21}^{-1} & 0 \\ 0 & V_{22}^{-1} \end{pmatrix}.
\end{equation*}
\end{proof}

A direct application of Prop.~\ref{prop:reparametrization.full.rank} guarantees that for every $\nu \geq 0$, one can enforce the full-rankness of $\begin{pmatrix} \wb{A} \\ \wb{V}_{21}^{-1} \end{pmatrix}$ by the one of $A - B V_{22} V_{21}^{-1}$.
\begin{corollary}
\label{co:reparametrization.full.rank}
For any $\nu \geq 0$, let $\wb{A}$ and $ \wb{V}^{-1}$ be the reparametrized matrices. If $A - B V_{22} V_{21}^{-1}$ is full rank, then $\ker(\wb{A}) \cap \ker(\wb{V}_{21}^{-1}) = \{ 0 \}$.
\end{corollary} 
%\begin{proof}
%For all $\nu \geq 0$, for all $x \in \ker(\wb{A}) \cap \ker(\wb{V}_{21}^{-1})$, one has:
%\begin{equation*}
%\begin{aligned}
%&&\wb{A} x = 0 \quad & \text{ and} &\quad \wb{V}_{21}^{-1}x = 0 \\
%&\Rightarrow& \quad A x  = \nu B (R + \nu I)^{-1} K_0 x \quad & \text{ and} &\quad V_{21}^{-1}x =  - \nu V_{22}^{-1} (R+\nu I)^{-1}K_0 x \\
%&\Rightarrow &\quad A x  = \nu B (R + \nu I)^{-1} K_0 x \quad & \text{ and} &\quad - V_{22} V_{21}^{-1}x =  \nu  (R+\nu I)^{-1}K_0 x \\
%&\Rightarrow &\quad A x  = - B V_{22} V_{21}^{-1}x \quad & \text{ and} &\quad - V_{22} V_{21}^{-1}x =  \nu  (R+\nu I)^{-1}K_0 x \\
%&\Rightarrow &x \in \ker \big( A + B V_{22} V_{21}^{-1} \big).
%\end{aligned}
%\end{equation*}
%As result, $\ker(\wb{A}) \cap \ker(\wb{V}_{21}^{-1}) \subset \ker \big( A + B V_{22} V_{21}^{-1} \big) = \{0 \}$.
%\end{proof}

As a result, for any $\nu > 0$, the linear reparametrization transforms the original problem into an instance similar to the one with $\nu = 0$ while preserving all the properties needed in the proof for the reparametrized matrices $\wb{A}$, $\wb{Q}$, $\wb{R}$ and $\wb{V}^{-1}$, namely the full-rankness of  $B$, $\ker(\wb{A}) \cap \ker(\wb{V_{21}}^{-1}) = \{ 0 \}$ and the positive definiteness of $\wb{Q},\wb{R},\wb{V}^{-1}$. Therefore, we only report the proof of Lem.~\ref{le:existence.closure.M} and~\ref{le:positivity.margin} for $\nu = 0$ and remove the dependency in $\nu$ in what follows to simplify the notation.

\subsection{Proof of Lem.~\ref{le:existence.closure.M}} 

The proof of Lem.~\ref{le:existence.closure.M} relies on the following result when $\nu = 0$.
\begin{proposition}
\label{p:finite.zeros.determinant}
Let $B$ be full column rank, $\ker(A) \cap \ker(V_{2,1}^{-1}) = \{ 0 \}$. Let $\tilde{\mu}$ be defined by Eq.~\eqref{eq:mutilde.definition}, then, for all $K$, $\det \Psi^{\tilde{\mu}}_K(z) = 0$ for finitely many $|z|=1$.
\end{proposition}
	
We prove Prop.~\ref{p:finite.zeros.determinant} by contradiction. Suppose that it exists some $K$ such that $\det \Psi^{\tilde{\mu}}_K(z) = 0$ for infinitely many $|z|=1$. Necessarily, it also holds for all $K$ (otherwise Thm.\ref{th:molinari75.2} holds). Then, it also holds for all $|z|=1$ since the function $\Psi$ is analytic on the unit circle. This allows us to pick a particular $\wb{K}$ for which we show the contradiction.
%
%
%This last statement can be easily checked using a specific control matrix $\wb{K} = \begin{pmatrix} 0 \\ A \end{pmatrix}$: for such $\wb{K}$, one has that 
%\begin{equation*}
%A(\wb{K}) = 0, \quad Q_{\tilde{\mu}}(\wb{K}) = Q_{\tilde{\mu}} + \tilde{\mu} A^\transp A, \quad N_{\tilde{\mu}}(\wb{K}) = - \tilde{\mu} \begin{pmatrix} V^{-1}_{2,1} \\ A \end{pmatrix},
%\end{equation*}
%where $V^{-1}_{2,1}$ is the off-diagonal block of $V^{-1}$. Then, using the parametrization $z = \cos(\theta) + i \sin(\theta)$ for all $\theta \in [0,2 \pi]$, one has:
%\begin{equation*}
%\det \Psi^{\tilde{\mu}}_{\wb{K}}(z) = \det \left ( \tilde{B}^T Q_{\tilde{\mu}}(\wb{K}) \tilde{B} + R_{\tilde{\mu}} + \cos(\theta) [ \tilde{B}^\transp N_{\tilde{\mu}}(\wb{K})^\transp + N_{\tilde{\mu}}(\wb{K})\tilde{B} ] \right) = 0,
%\end{equation*}
%which is polynomial in $\cos(\theta)$ with infinitely many roots, and hence which is zero everywhere (for all $\theta \in [0,2\pi]$). Further, necessarily, $\det ( \tilde{B}^T Q_{\tilde{\mu}}(\wb{K}) \tilde{B} + R_{\tilde{\mu}}) = 0$ (taking $\theta = \pi/2$). Thus, since $\tilde{B}^T Q_{\tilde{\mu}}(\wb{K}) \tilde{B} + R_{\tilde{\mu}} \succcurlyeq 0$, there exists $\wt{u}_0 \neq 0 \in \mathbb{R}^{n+d}$ such that 
%\begin{equation}
%\label{eq:u0.definition1}
%\wt{u}_0^\transp ( \tilde{B}^T Q_{\tilde{\mu}}(\wb{K}) \tilde{B} + R_{\tilde{\mu}})  \wt{u}_0 = 0.
%\end{equation}
%Finally, necessarily for such $\wt{u}_0$, 
%\begin{equation}
%\label{eq:u0.condition2}
%\wt{u}_0^\transp ( \tilde{B}^\transp N_{\tilde{\mu}}(\wb{K})^\transp + N_{\tilde{\mu}}(\wb{K})\tilde{B} )  \wt{u}_0 = 0
%\end{equation}
%otherwise there exists $\theta \in [0, 2\pi]$ such that $\wt{u}_0^\transp \det \Psi^{\tilde{\mu}}_{\wb{K}}(z)  \wt{u}_0 > 0$ which is impossible. As a result, let 
%\begin{equation}
%\label{eq:zero.eigenvector.set}
%\mathcal{U} := \{ \wt{u} \in \mathbb{R}^{n+d} \neq 0 \text{ satisfying Eq.~\eqref{eq:u0.definition1} and~\eqref{eq:u0.condition2}} \},
%\end{equation}
%the previous reasoning ensures that $\mathcal{U}$ non-empty. Further, this set satisfies the following property:


\begin{property}
\label{p:ker.set}
Let $\wb{K} = \begin{pmatrix} 0 \\  - A \end{pmatrix}$ and let $\ker(A) \cap \ker(V_{2,1}^{-1}) = \{ 0 \}$ . Suppose that $\det \Psi^{\tilde{\mu}}_{\wb{K}}(z) = 0$ for infinitely many $|z|=1$ and let $\mathcal{U} = \{ \wt{u} \neq 0 \text{ s.t. } \wt{u}^\transp \Psi^{\tilde{\mu}}_{\wb{K}}(z) \wt{u} = 0 \text{ for all } |z| = 1 \}$. Then, $\mathcal{U} \subset \text{Ker}(\tilde{B})$.
\end{property}
%
\begin{proof}[Proof of Property.~\ref{p:ker.set}]
By assumption, $\wt{u}^\transp \Psi^{\tilde{\mu}}_{\wb{K}}(z) \wt{u} = 0$ for all $|z|=1$ and all $\wt{u} \in \mathcal{U}$. Hence by continuity, for all $\epsilon > 0$, there exists $\eta >0$ such that $\wt{u}^\transp \Psi^{\tilde{\mu} - \eta}_{\wb{K}}(z) \wt{u} < \epsilon$ for all $|z|=1$ and all $\wt{u} \in \mathcal{U}$. Further, from [Molinari, 1975, Lem.4], we have that 
\begin{equation}
\label{eq:molinari.lem4}
\begin{aligned}
\Psi^{\tilde{\mu} - \eta}_{\wb{K}}(z) = \Delta(z^{-1}) D_{\tilde{\mu} - \eta} \Delta(z) \quad\text{ where } \quad \Delta(z) = I + z  D_{\tilde{\mu} - \eta}^{-1} N_{\tilde{\mu} - \eta}(\wb{K}) \tilde{B} \quad \text{ and } \quad D_{\tilde{\mu} - \eta} = R_{\tilde{\mu} - \eta} + \tilde{B}^\transp P_{\tilde{\mu} - \eta} \tilde{B}.
\end{aligned}
\end{equation}
%
Thus, for all $\wt{u} \in \mathcal{U}$,
\begin{equation*}
\begin{aligned}
\wt{u}^\transp \Psi^{\tilde{\mu} - \eta}_{\wb{K}}(z) \wt{u} &= \wt{u}^\transp [ D_{\tilde{\mu} - \eta} + \tilde{B}^\transp N_{\tilde{\mu} - \eta}(\wb{K}) ^\transp D_{\tilde{\mu} - \eta}^{-1} N_{\tilde{\mu} - \eta}(\wb{K})  \tilde{B} ] \wt{u} + \cos(\theta) \wt{u}^\transp [\tilde{B}^\transp N_{\tilde{\mu} - \eta}(\wb{K}) ^\transp + N_{\tilde{\mu} - \eta}(\wb{K})  \tilde{B}] \wt{u} \\
\wt{u}^\transp \Psi^{\tilde{\mu} - \eta}_{\wb{K}}(i) \wt{u} &= \wt{u}^\transp [ D_{\tilde{\mu} - \eta} + \tilde{B}^\transp N_{\tilde{\mu} - \eta}(\wb{K}) ^\transp D_{\tilde{\mu} - \eta}^{-1} N_{\tilde{\mu} - \eta}(\wb{K})  \tilde{B} ] \wt{u}.
\end{aligned}
\end{equation*}
Finally, by construction $\tilde{\mu} - \eta \in [0,\wt{\mu})$, so $D_{\tilde{\mu} - \eta} \succ 0$ and $\|D_{\tilde{\mu} - \eta}\|_2 \leq c$, where $c$ is a finite constant independent of $\epsilon$. As a result,
\begin{equation*}
\begin{aligned}
&\wt{u}^\transp [ \tilde{B}^\transp N_{\tilde{\mu} - \eta}(\wb{K}) ^\transp D_{\tilde{\mu} - \eta}^{-1} N_{\tilde{\mu} - \eta}(\wb{K})  \tilde{B} ] \wt{u} \leq \wt{u}^\transp \Psi^{\tilde{\mu} - \eta}_{\wb{K}}(z) \wt{u} < \epsilon\\
&\Rightarrow \quad \wt{u}^\transp [ \tilde{B}^\transp N^\transp_{\tilde{\mu} - \eta}(\wb{K})  N_{\tilde{\mu} - \eta}(\wb{K})  \tilde{B} ] \wt{u} < \epsilon/c.
\end{aligned}
\end{equation*}
Notice that since $\ker(A) \cap \ker(V_{2,1}^{-1}) = \{ 0 \}$, $N_{\tilde{\mu} - \eta}(\wb{K})^\transp  N_{\tilde{\mu} - \eta}(\wb{K}) = \big(V_{2,1}^{-1}\big)^\transp V_{2,1}^{-1} + A^\transp A   \succ 0$. This implies that $\wt{u}\in\text{Ker}(\tilde{B})$ by taking $\epsilon \rightarrow 0$.\\
\end{proof}
%
Equipped with this characterization, we are now ready to prove Prop.~\ref{p:finite.zeros.determinant}. Let $\wb{K}$ be defined as in Property.~\ref{p:ker.set}. A similar reasoning guarantees  that it exists at least one $\wt{u} \in \mathcal{U} \neq 0$ such that for all $\epsilon > 0$, there exists $\eta >0$ such that
\begin{equation}
\label{eq:almost.null.D}
0 <\wt{u}^\transp \Psi^{\tilde{\mu} - \eta}_{\wb{K}}(z) \wt{u} < \epsilon,
\end{equation}
Further, using Eq.~\ref{eq:molinari.lem4} and that $\mathcal{U} \subset \ker(\wt{B})$, Eq.~\ref{eq:almost.null.D} directly implies that $0 <\wt{u}^\transp D_{\tilde{\mu} - \eta} \wt{u} < \epsilon$. Notice that $D_{\tilde{\mu} - \eta}= R_{\tilde{\mu} - \eta} + \tilde{B}^\transp P_{\tilde{\mu} - \eta} \tilde{B}$ do not depend on $\bar{K}$. Since $\wt{u} = (u^\transp, w^\transp)^\transp \in \ker(\wt{B})$, 
\begin{equation*}
\wt{u}^\transp D_{\tilde{\mu} - \eta} \begin{pmatrix} 0 \\ I \end{pmatrix} = \wt{u}^\transp R_{\tilde{\mu} - \eta} \begin{pmatrix} 0 \\ I \end{pmatrix} = (\tilde{\mu} - \eta) w \quad \quad \text{ and } \quad \quad w = - B u.
\end{equation*} 
Further, since $B$ is full column rank and $\wt{u} \neq 0$, we have that $\|w\| \geq c >0$. Thus, 
\begin{equation*}
(\tilde{\mu} - \eta) \|w\| \leq \| \wt{u}^\transp D_{\tilde{\mu} - \eta}^{1/2}\| \|D_{\tilde{\mu} - \eta}^{1/2} \| \|I\| \leq \sqrt{\epsilon} \sqrt{\|D_{\tilde{\mu} - \eta}\|}.
\end{equation*}
Since $\tilde{\mu} > 0$  and $\|D_{\mu}\| < \infty$ for all $\mu \leq \wt{\mu}$, taking $\epsilon \rightarrow 0$ leads to the contradiction.



%
%Now recall that, by definition:
%\begin{equation}
%\label{eq:K.equivalent.definition.1}
%K_{\tilde{\mu} - \eta}  = - D^{-1} \big( \tilde{B}^\transp P_{\tilde{\mu} - \eta} A + N_{\tilde{\mu} - \eta}\big) 
%\end{equation}
%which for any controller $K$ can be rewritten as:
%\begin{equation}
%\label{eq:K.equivalent.definition.2}
%K_{\tilde{\mu} - \eta}  = - D^{-1} \big( \tilde{B}^\transp P_{\tilde{\mu} - \eta} A(K) + N_{\tilde{\mu} - \eta}(K)\big) + K.
%\end{equation}
%Eq.~\ref{eq:K.equivalent.definition.2} can be easily checked using $A(K) = A + B K$ and $N_{\tilde{\mu} - \eta}(K) = N_{\tilde{\mu} - \eta} + R_{\mu - \eta} K$. 	
%From Eq.~\ref{eq:K.equivalent.definition.1} and Eq.~\ref{eq:K.equivalent.definition.2} applied at $K = \begin{pmatrix} 0 \\ - I \end{pmatrix}$, one has:
%\begin{equation*}
%\begin{aligned}
%D K_{\tilde{\mu} - \eta} &= - \big( \tilde{B}^\transp P_{\tilde{\mu} - \eta} A + N_{\tilde{\mu} - \eta}\big) = - \tilde{B}^\transp P_{\tilde{\mu} - \eta} A + (\tilde{\mu} - \eta)  \begin{pmatrix} V_{2,1}^{-1} \\ 0 \end{pmatrix},\\
%D K_{\tilde{\mu} - \eta} &= - \big( \tilde{B}^\transp P_{\tilde{\mu} - \eta} A(K) + N_{\tilde{\mu} - \eta}(K)\big) + D \wb{K} = -  \tilde{B}^\transp P_{\tilde{\mu} - \eta} A(K) +  (\tilde{\mu} - \eta)  \begin{pmatrix} V_{2,1}^{-1} \\ I \end{pmatrix} + D  \begin{pmatrix} 0 \\ - I \end{pmatrix}.
%\end{aligned}
%\end{equation*}
%Hence, for all $\wt{u} \in \mathcal{U}$,
%\begin{equation}
%\label{eq:distinc.case.K}
%\begin{aligned}
%\wt{u}^\transp D K_{\tilde{\mu} - \eta}  &= (\tilde{\mu} - \eta)  \wt{u}^\transp  \begin{pmatrix} V_{2,1}^{-1} \\ 0 \end{pmatrix}, \\
%\wt{u}^\transp D K_{\tilde{\mu} - \eta}  &= (\tilde{\mu} - \eta)  \wt{u}^\transp \begin{pmatrix} V_{2,1}^{-1} \\ I \end{pmatrix} + u^\transp D  \begin{pmatrix} 0 \\ - I \end{pmatrix}.
%\end{aligned}
%\end{equation}
%%
%Substracting those two equalities, one gets, for all $\wt{u}\in\mathcal{U}$:
%\begin{equation*}
%(\tilde{\mu} - \eta)  \wt{u}^\transp \begin{pmatrix} 0 \\ I \end{pmatrix} = \wt{u}^\transp D  \begin{pmatrix} 0 \\ I \end{pmatrix}.
%\end{equation*}
%Using $\wt{u}^\transp = (u, w)$, taking the norm and using Eq.~\ref{eq:almost.null.D}, one has $(\tilde{\mu} - \eta) \|w\| \leq \| \wt{u}^\transp D^{1/2}\| \|D^{1/2} \| \|I\| \leq \sqrt{\epsilon} \sqrt{\|D\|}$.
%Finally, from $\mathcal{U} \subset \text{Ker}(\tilde{B})$, $w = - B u$. Since $B$ is full column rank and $\wt{u} \neq 0$, we have that $\|w\| \geq c >0$ and taking $\epsilon \rightarrow 0$ leads to the contradiction.
%\end{proof}

\subsection{Proof of Lem.~\ref{le:positivity.margin}}
Now that existence and uniqueness of $P_\mu$ for all $\mu \leq \wt{\mu}$ are guaranteed, we explicit a lower bound on $D_\mu$ for \textit{some} $\mu \leq \tilde{\mu}$. Notice that $D_\mu$ is not affected by the reparametrization, and hence the lower bound for $\nu=0$ directly translates in a lower bound for the original problem for any $\nu \geq 0$.

\begin{lemma}\label{le:positivity.margin}
Let $B$ be full column rank and $\ker(A) \cap \ker(V_{2,1}^{-1}) = \{ 0 \}$. For all $\mu \leq \tilde{\mu}$ such that $\|K_\mu\|_2 \leq c < \infty$, $D_\mu \succcurlyeq \alpha I$, where 
\begin{equation*}
\begin{aligned}
&\alpha =  \min\left(  \frac{c_2}{(c_1 c_2)^{n+d}} \min \left( c_3, \frac{\wb{\epsilon} \alpha_{\min}}{c_2} \right),\frac{\lambda_{\min}(H)}{4 \max\big(2,1 + 2 \|B\|_2^2)}\right), \\
&c_1 = 1 + \Big( (\|A\|_2 + c )\|\tilde{B}\|_2 \Big)^2; \quad c_2 =\max\big( \lambda_{\max}(R), \tilde{\mu}\big) + (D + n \tilde{\mu}) \|\tilde{B}\|_2^2; \quad c_3 = (\mu_+ \alpha_{\min}(B))/2,\\
&\alpha_{\min} = \sigma_{\min}\big( N_{\mu}(\wb{K}) \big);\quad \alpha_{\min}(B) = \frac{\sigma_{\min}(B)^2}{2 (2 + \sigma_{\min}(B)^2)}; \quad 
\wb{\epsilon} = \min \left( \alpha_{\min}(B),  \frac{\mu_+ \alpha_{\min}(B)}{2 (D + n \tilde{\mu}))}\right),\\
&\mu_+ \text{ is the solution of } \lambda_{\min}(H_{\mu_+}) = \lambda_{\min} \left( H - \mu_+ V^{-1} \right) = 1/2 \lambda_{\min}(H).
\end{aligned}
\end{equation*}
\end{lemma}

The proof of Lem.~\ref{le:positivity.margin} relies on the following intermediate results:
\begin{proposition}\label{prop:bounded.popov.determinant}
For all $\mu \leq \tilde{\mu}$, if $\|K_\mu\|_2 \leq c$, $$\det\big( \Psi_{\wb{K}}^\mu(i) \big) \leq \det\big( D_\mu\big) c_1^{n+d}$$ where $\wb{K} = \begin{pmatrix} 0 \\  - A \end{pmatrix}$ and 
$c_1 = 1 + \Big( (\|A\|_2 + c )\|\tilde{B}\|_2 \Big)^2$.
\end{proposition}

\begin{corollary}\label{co:bounded.popov.determinant}
For all $\mu \leq \tilde{\mu}$, if $\|_\mu\|_2 \leq c$, let $v_{\min}$ be the eigenvector associated with the minimum eigenvalue of $\Psi_{\wb{K}}^\mu(i)$, then,
\begin{equation*}
\| \tilde{B} v_{\min} \|_2^2 \leq \frac{c_1 c_2}{\alpha_{\min}} \det\big( D_\mu\big) ^{1/(n+d)},
\end{equation*} 
where $c_2 = \max\big( \lambda_{\max}(R), \mu\big) + (D + n \mu) \|\tilde{B}\|_2^2$ and $\alpha_{\min} = \sigma_{\min}\big( N_{\mu}(\wb{K}) \big)$. 
\end{corollary}

\begin{proposition}\label{prop:positivity.kerB}
For all $\mu_+ \geq \mu \leq \tilde{\mu}$, if $\|K_\mu\|_2 \leq c$. For all $\|v\|=1$ such that $\|\tilde{B} v \|_2^2 \leq \bar{\epsilon}$, $v^\transp D_\mu v \geq c_3$, where
\begin{equation*}
c_3 = (\mu_+ \alpha_{\min}(B))/2;  \quad \quad \alpha_{\min}(B)^2 = \frac{\sigma_{\min}(B)^2}{2 (2 + \sigma_{\min}(B)^2)}; \quad \quad \bar{\epsilon} = \min \left( \alpha_{\min}(B),  \frac{\mu_+ \alpha_{\min}(B)}{2 (D + n\mu))}\right).\\
\end{equation*}
\end{proposition}
We first prove all the intermediate results and then proceed with the proof of Lem.~\ref{le:positivity.margin}.

\paragraph{Proof of Prop.~\ref{prop:bounded.popov.determinant}.} From~\citep{molinari1975}, we have that, for all $|z|=1$,
\begin{equation*}
\Psi_{\wb{K}}^\mu(z) = \big( I + (K_\mu - \wb{K}) z^{-1} \tilde{B} \big)^\transp \Psi_{K_\mu}^\mu(z)  \big( I + (K_\mu - \wb{K}) z \tilde{B} \big),
\end{equation*}
and that $\Psi_{K_\mu}^\mu(z) = D_\mu$. Thus, 
\begin{equation*}
\begin{aligned}
\det\big( \Psi_{\wb{K}}^\mu(i) \big) &= \det(D_\mu) \det\Big( \big( I + i^{-1} (K_\mu - \wb{K}) \tilde{B} \big)^\transp  \big( I + i (K_\mu - \wb{K}) \tilde{B} \big) \Big) \\
&\leq \det(D_\mu) \big( 1 + \| (K_\mu - \wb{K}) \tilde{B} \|_2^2 \big)^{n+d} \leq \det(D_\mu)  \big( 1 + (c + \|A\|) \|\tilde{B} \|_2^2 \big)^{n+d}.
\end{aligned}
\end{equation*}

\paragraph{Proof of Cor.~\ref{co:bounded.popov.determinant}.} From Eq.~\ref{eq:molinari.lem4}, $\lambda_{\min}\big( \Psi_{\wb{K}}^\mu(i) ) \geq v_{\min}^\transp N_\mu(\wb{K})^\transp  \tilde{B}^\transp D_\mu^{-1} N_\mu(\wb{K}) \tilde{B} v_{\min}$.
%\begin{equation*}
%\lambda_{\min}\big( \Psi_{\wb{K}}^\mu(i) ) \geq v_{\min}^\transp N_\mu(\wb{K})^\transp  \tilde{B}^\transp D_\mu^{-1} N_\mu(\wb{K}) \tilde{B} v_{\min}.
%\end{equation*}
Further, since $\Tr( P_\mu ) \leq D$ and $P_\mu + \mu I \succ 0$, one has $\|P_\mu\|_2 \leq (D + n \mu)$ which implies that $D_\mu \preccurlyeq c_2 I$. Thus,
\begin{equation*}
\lambda_{\min}\big( \Psi_{\wb{K}}^\mu(i) ) \geq \frac{\alpha_{\min}}{c_2} \| \tilde{B} v_{\min} \|_2 \quad \quad \Rightarrow \quad \quad \| \tilde{B} v_{\min} \|^2_2 \leq \frac{c_1 c_2}{\alpha_{\min}} \det( D_\mu)^{1/(n+d)}.
\end{equation*}

\paragraph{Proof of Prop.~\ref{prop:positivity.kerB}.} Let $v^\transp = (u^\transp \hspace{1mm} w^\transp)$. From $\|\tilde{B} v \|_2 \leq \alpha_{\min}$ and $\|v\|=1$ we have that 
\begin{equation*}
\begin{aligned}
\|B u \| - \|w\| \leq \|\tilde{B} v \| \leq \alpha_{\min} \quad &\Rightarrow \quad  \sigma_{\min}(B) \sqrt{1 - \|w\|^2} = \sigma_{\min}(B) \|u\| \leq \alpha_{\min} + \|w\| \\
&\Rightarrow \quad  \sigma_{\min}(B)^2 (1 - \|w\|^2 ) \leq 2 \alpha_{\min}^2 + 2 \|w\|^2 \\
&\Rightarrow \quad  \|w\|^2 \geq  \frac{\sigma_{\min}(B)^2 - 2 \alpha_{\min}^2 }{ 2 + \sigma_{\min}(B)^2} \geq \alpha_{\min}^2\\
 &\Rightarrow \quad  \|w\| \geq  \alpha_{\min}.
\end{aligned}
\end{equation*}
Further, from $D_\mu \begin{pmatrix} 0 \\ I \end{pmatrix} = \mu \begin{pmatrix} 0 \\ I \end{pmatrix} + \tilde{B}^\transp P_\mu$, one gets:
\begin{equation*}
\begin{aligned}
v^\transp D_\mu  \begin{pmatrix} 0 \\ I \end{pmatrix} = \mu w^\transp + v^\transp  \tilde{B}^\transp P_\mu \quad &\Rightarrow \quad \| P_\mu \tilde{B} v + \mu w\| \leq \|D^{1/2} v \| \|D^{1/2}\| \leq \sqrt{v^\transp D v} c_2 \\
&\Rightarrow \quad \mu \|w\| - \|P_\mu\|_2 \bar{\epsilon} \leq  \sqrt{v^\transp D v} c_2 \\
&\Rightarrow \quad \mu_+ \alpha_{\min} - (D + n \mu) \bar{\epsilon} \leq  \sqrt{v^\transp D v} c_2 \\
\end{aligned}
\end{equation*}

\paragraph{Proof of Lem.~\ref{le:positivity.margin}.} To provide a lower bound on $D_\mu$, we distinguish the case when $\mu < \mu_+$ and $\mu \geq \mu_+$, where $\mu_+$ set such that $\lambda_{\min}(H_{\mu_+}) = \lambda_{\min} \left( H - \mu_+ V^{-1} \right) = 1/2 \lambda_{\min}(H)$.
\begin{enumerate}
\item When $\mu < \mu_+$, $H_\mu \succ H_{\mu_+}$ is psd and hence  $P_\mu \succ 1/2 \lambda_{\min}(H) I $. Following a similar path as for the proof of Prop.~\ref{prop:positivity.kerB}, for any $\|v\|=1$, $v^\transp = (u^\transp \hspace{1mm} w^\transp)$, if $\| \tilde{B} v \| \leq 1/2$, then
\begin{equation*}
\|B u + w \| \leq 1/2 \quad \Rightarrow \quad \|w\|^2 \leq 1/2 + 2 \|B\|_2^2 \|u\|^2 \quad \Rightarrow \quad 1/2 \leq (1 + 2 \|B\|_2^2) \|u\|^2,
\end{equation*}
and 
\begin{equation*}
v^\transp D_\mu v \geq u^\transp (R - \mu V_{22}^{-1}) u \geq 1/2 \lambda_{\min}(H) \|u\|^2 \geq \frac{\lambda_{\min}(H)}{4 (1 + 2 \|B\|_2^2) }.
\end{equation*}
Otherwise, if $\|\tilde{B} v \| \geq 1/2$ then $v^\transp D_\mu v \geq v^\transp \tilde{B}^\transp P_\mu \tilde{B} v \geq 1/2 \lambda_{\min}(H) \|\tilde{B} v \|^2 \geq 1/8 \lambda_{\min}(H)$.
As a result, 
\begin{equation*}
D_\mu \succcurlyeq \frac{\lambda_{\min}(H)}{4 \max\big(2,1 + 2 \|B\|_2^2)}.
\end{equation*}
\item When $\mu \geq \mu_+$, if $\lambda_{\min}(D_\mu) \leq c_2 \left(\frac{\bar{\epsilon} \alpha_{\min}}{c_1 c_2^2}\right)^{n+d}$ then $\det(D_\mu) \leq \left(\frac{\bar{\epsilon} \alpha_{\min}}{c_1 c_2}\right)^{n+d} $ and applying Cor.~\ref{co:bounded.popov.determinant} and Prop.~\ref{prop:positivity.kerB}, one gets that $v_{\min}^\transp D_\mu v_{\min} \geq c_3$. However, from $\Psi_{\wb{K}}^\mu(i) \succ D_\mu$, one gets that 
$v_{\min}^\transp \Psi_{\wb{K}}^\mu(i) v_{\min} > v_{\min}^\transp D_\mu v_{\min} \geq c_3$ which imlies that $ \det\big( \Psi_{\wb{K}}^\mu(i) \big) \geq c_3^{n+d}$. As a result, 
$\det(D_\mu) \geq \big( c_3 / c_1)^{n+d}$ and $\lambda_{\min}(D_\mu) \geq c_2  ( c_3 / c_1 c_2)^{n+d}$. Thus, \\
either 
\begin{equation*}
\lambda_{\min}(D_\mu) \leq c_2 \left(\frac{\bar{\epsilon} \alpha_{\min}}{c_1 c_2^2}\right)^{n+d} \quad \Rightarrow \quad \lambda_{\min}(D_\mu) \geq c_2  ( c_3 / c_1 c_2)^{n+d},
\end{equation*}
either 
\begin{equation*}
\lambda_{\min}(D_\mu)  \geq c_2 \left(\frac{\bar{\epsilon} \alpha_{\min}}{c_1 c_2^2}\right)^{n+d} .
\end{equation*}
\end{enumerate}
Plugging everything together, one gets:
\begin{equation*}
D_\mu \succcurlyeq \min\left(  \frac{c_2}{(c_1 c_2)^{n+d}} \min \left( c_3, \frac{\wb{\epsilon} \alpha_{\min}}{c_2} \right),\frac{\lambda_{\min}(H)}{4 \max\big(2,1 + 2 \|B\|_2^2)}\right). 
\end{equation*}








==> sec_ofu.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[t]
%\begin{center}
%\vspace{-0.1in}
%\bookboxx{
%\begin{small}
%    \begin{algorithmic}[1]
%        \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%        \renewcommand{\algorithmicensure}{\textbf{Output:}}
%        \vspace{-0.02in}
%        \REQUIRE $\Theta_0$, $V_0 = \lambda I$, $\delta$, $T$, $t_0 = 0$
%        %\STATE Set $\delta' = \delta/(8T)$ and $\beta_t = \beta_t(\delta')$ according to Eq.~\ref{eq:lqr.beta-definition}
%        \FOR{$k = \{1, \dots\}$}
%            \STATE Compute the confidence interval $\C_k$ as in~\eqref{eq:conf.interval}
%        	\STATE Compute $\wt\theta_k$ solving \eqref{eq:ofu.real}
%        	\WHILE{$\det(V_t) < 2 \det(V_{t_k})$}
%             \STATE Execute control  $u_t = K(\wt\theta_{t_k}) x_t$
%            \STATE  Observe state $x_{t+1}$ and cost $c_t = c(x_t,u_t)$
%            \STATE  Update $V_{t+1}$ and $\wh\theta_{t+1}$ as in~\eqref{eq:lq-least.square} and $t=t+1$
%            \ENDWHILE
%        \ENDFOR
%
%    \end{algorithmic}
%    \vspace{-0.1in}
%    \caption{\small The \ofu algorithm for LQ systems.}
%    \label{alg:lq.ofu}
%\end{small}
%}
%\vspace{-0.2in}
%\end{center}
%\end{figure}

\textbf{Optimism in LQR.} \citet{abbasi2011regret} proposed to integrate the optimism-in-face-of-uncertainty principle into LQR by exploiting the confidence interval defined in Prop.~\ref{p:concentration} to identify the parameter $\wt\theta$ minimizing the average cost $J(\theta)$. The algorithm %(see Fig.~\ref{alg:lq.ofu}) 
receives as input a set $\Theta_0$ and proceeds through episodes $k=1,2,\ldots$ and at the beginning of each episode it computes a parameter
%
\begin{align}\label{eq:ofu.real}
\wt\theta_k = \arg\min_{\theta \in \mathcal{C}_k \cap \Theta_0} J(\theta).
\end{align}
%
where $t_k$ is the step at which episode $k$ begins and the constrained set $\mathcal{C}_k$ is defined as									
%
\begin{align}\label{eq:conf.interval}
\mathcal{C}_k = \mathcal{C}(\beta_{t_k}, V_{t_k}) := \{\theta: \| \theta - \wh{\theta}_{t_k} \|_{V_{t_k}} \leq \beta_{t_k}\},
\end{align}
%
where $\beta_t = \beta_t(\delta/4T)$ is defined as Eq.~\ref{eq:lqr.beta-definition} with $\theta_0 = 0$. Notice that the term $\Tr(\theta_*\theta_*^\transp)$ is unknown and in $\beta_t$ we replace it by an upper-bound $S$ derived from $\Theta_0$. %\citet{abbasi2011regret} also showed that, in practice, it is enough to solve problem~\eqref{eq:ofu.real} up to an error $1/\sqrt{t_k}$, i.e., compute a parameter $\wt\theta_k$ such that $J(\wt\theta_k) \leq \min_{\theta \in \mathcal{C}_k} J(\theta) + 1/\sqrt{t_k}$. 
The optimal control $K(\wt\theta_t)$ is computed (see~\eqref{eq:lqr.solution}) and the corresponding policy is executed until $\det(V_t) \geq 2\det(V_{t_k})$. %Under suitable stability condition on the state process $\{x_t\}_t$, it is easy to show that the episode stopping condition leads a number of episodes that grows at most logarithmically with the number of steps.
%. Let $\mathcal{K}_{\epsilon} = \{K: \|K-K(\theta_0)\} \leq \epsilon\}$ be smallest set of controllers that contains all the optimal controllers $K(\theta)$ with $\theta\in\Theta_0$. More formally, $\epsilon = \min\{\epsilon: \forall \theta\in\Theta_0, K(\theta)\in\mathcal{K}_\epsilon\}$

